Towards Realistic Mechanisms That Incentivize Federated Participation and Contribution

Edge device participation in federating learning (FL) is typically studied through the lens of device-server communication (e.g., device dropout) and assumes an undying desire from edge devices to participate in FL. As a result, current FL frameworks are flawed when implemented in realistic settings, with many encountering the free-rider dilemma. In a step to push FL towards realistic settings, we propose RealFM: the first federated mechanism that (1) realistically models device utility, (2) incentivizes data contribution and device participation, (3) provably removes the free-rider dilemma, and (4) relaxes assumptions on data homogeneity and data sharing. Compared to previous FL mechanisms, RealFM allows for a non-linear relationship between model accuracy and utility, which improves the utility gained by the server and participating devices. On real-world data, RealFM improves device and server utility, as well as data contribution, by over 3 and 4 magnitudes respectively compared to baselines.

==> figures/old/accuracy-plots-16.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-16device-cifar10.png}
   \label{fig:cifar-acc-16}
   \caption{16 Devices on CIFAR-10.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-16device-mnist.png}
   \label{fig:mnist-acc-16}
   \caption{16 Devices on MNIST.}
\end{subfigure}
\caption{\textbf{Test Accuracy for Local versus Federated Training on CIFAR-10 and MNIST.} As expected, FedAvg greatly outperforms Local Training by nearly $20$\% for $16$ devices respectively on CIFAR-10. MNIST is an easier dataset to classify, so both Local Training and FedAvg do great jobs at classifying digits. However, FedAvg does perform at a $99+$\% accuracy whereas Local Training sits around $98$\%. While this may seem to be a small gap, the utility gained by having a nearly perfect classification scheme is much greater than that having only $98$\%.}
\label{fig:acc-plots-16}
\end{figure}

==> figures/old/accuracy-plots-8.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-8device-cifar10.png}
   \label{fig:cifar-acc-8} 
   \caption{8 Devices on CIFAR-10.}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-8device-mnist.png}
   \label{fig:mnist-acc-8} 
   \caption{8 Devices on MNIST.}
\end{subfigure}
\caption{\textbf{Test Accuracy for Local versus Federated Training on CIFAR-10 and MNIST.} As expected, FedAvg greatly outperforms Local Training by nearly $14$\% for $8$ devices respectively on CIFAR-10. MNIST is an easier dataset to classify, so both Local Training and FedAvg do great jobs at classifying digits. However, FedAvg does perform at a $99+$\% accuracy whereas Local Training sits around $98$\%. While this may seem to be a small gap, the utility gained by having a nearly perfect classification scheme is much greater than that having only $98$\%.}
\label{fig:acc-plots-8}
\end{figure}

==> figures/old/cifar-accuracy-plots.tex <==
\begin{figure}[H]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-8device-cifar10.png}
   \caption{Test Accuracy for 8 Devices.}
   \label{fig:cifar-acc-8} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-16device-cifar10.png}
   \caption{Test Accuracy for 16 Devices.}
   \label{fig:cifar-acc-16}
\end{subfigure}
\caption{\textbf{Test Accuracy for Local versus Federated Training on CIFAR-10.} As expected, FedAvg greatly outperforms Local Training by nearly $14$\% and $20$\% for $8$ and $16$ devices respectively.}
\label{fig:cifar-acc}
\end{figure}

==> figures/old/cifar-server-16.tex <==
\begin{figure}[t]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-utility-16devices.png}
   \caption{Server Utility Comparison.}
   \label{fig:server-u-16} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-data-produced-16devices.png}
   \caption{Average Data Contribution Comparison.}
   \label{fig:server-g-16}
\end{subfigure}
\caption{\textbf{Improved Server Utility on CIFAR-10.} \realfm increases central server utility (\ref{fig:server-u-16}) on CIFAR-10 for $16$ devices compared to relevant baselines. Tasked with non-linear (and possibly non-uniform) payoff functions, \realfm achieves over $15$x more utility than a FL version of \citep{karimireddy2022mechanisms} (denoted as \textsf{Linear} \realfm). \realfm incentivizes devices to produce over $250$\% more data points (\ref{fig:server-g-16}) than they would on their own.}
\label{fig:cifar-server-16}
\end{figure}


==> figures/old/cifar-server-8.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-utility-8devices.png}
   \caption{Server Utility Comparison.}
   \label{fig:server-u-8}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-data-produced-8devices.png}
   \caption{Average Data Contribution Comparison.}
   \label{fig:server-g-8}
\end{subfigure}
\caption{\textbf{Server Utility for $8$ Devices on CIFAR-10.}}
\label{fig:cifar-server-8}
\end{figure}


==> figures/old/data-contribution-comparison-16-old.tex <==
\begin{figure*}[!t]
\centering
%\hfill
   \begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-16devices.png}
   \label{fig:cifar-16-data} 
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-16devices-noniid0.6.png}
   \label{fig:cifar-16-0.6-data}
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-16devices-noniid0.3.png}
   \label{fig:cifar-16-0.3-data}
\end{subfigure}
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-16devices.png}
   \label{fig:mnist-16-data} 
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-16devices-noniid0.6.png}
   \label{fig:mnist-16-0.6-data}
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-16devices-noniid0.3.png}
   \label{fig:mnist-16-0.3-data}
\end{subfigure}
\vspace{-6mm}
\caption{\textbf{Increased Federated Contribution on CIFAR-10 \& MNIST.} \realfm incentivizes devices to use more local data during federated training on CIFAR-10 (top row) and MNIST (bottom row) for $16$ devices compared to relevant baselines. \realfm achieves upwards of 4 magnitudes more federated contributions than \textsc{Linear} \realfm across both uniform and various heterogeneous Dirichlet data distributions (left: uniform, center: D-0.6, right: D-0.3) as well as non-uniform costs (C) and accuracy payoff functions (P).}
\label{fig:data-contribution-comparsion-16}
\end{figure*}

==> figures/old/data-contribution-comparison-8-old.tex <==
\begin{figure*}[!ht]
\centering
%\hfill
   \begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-8devices.png}
   \label{fig:cifar-8-data} 
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-8devices-noniid0.6.png}
   \label{fig:cifar-8-0.6-data}
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-cifar10-8devices-noniid0.3.png}
   \label{fig:cifar-8-0.3-data}
\end{subfigure}
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-8devices.png}
   \label{fig:mnist-8-data} 
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-8devices-noniid0.6.png}
   \label{fig:mnist-8-0.6-data}
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/data-contributions/realfm-average-device-contribution-mnist-8devices-noniid0.3.png}
   \label{fig:mnist-8-0.3-data}
\end{subfigure}
\caption{\textbf{Increased Federated Contribution on CIFAR-10 \& MNIST.} \realfm incentivizes devices to use more local data during federated training on CIFAR-10 (top row) and MNIST (bottom row) for $8$ devices compared to relevant baselines. \realfm achieves upwards of 4 magnitudes more federated contributions than a FL version of \citet{karimireddy2022mechanisms}, denoted as \textsc{Linear} \realfm, across both uniform and various heterogeneous Dirichlet data distributions (left: uniform, center: D-0.6, right: D-0.3) as well as non-uniform costs (C) and accuracy payoff functions (P).}
\label{fig:data-contribution-comparsion-8}
\end{figure*}

==> figures/old/device-utility-16.tex <==
\begin{figure}[!htbp]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/device-utility/realfm-device-utility-16device.png}
   \caption{Average Device Utility Gained on CIFAR-10.}
   \label{fig:device-u-16-cifar} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/device-utility/realfm-device-utility-16device-mnist.png}
   \caption{Average Device Utility Gained on MNIST.}
   \label{fig:device-u-16-mnist}
\end{subfigure}
\caption{\textbf{Improved Device Utility on Real-World Data.} \realfm improves device utility derived from accuracy by upwards of $6$x and \textit{$4$ magnitudes} on CIFAR-10 and MNIST respectively. Only uniform experiments are run to save space since the non-uniform results are nearly identical.}
\label{fig:util-device-16}
\end{figure}

==> figures/old/device-utility-8.tex <==
\begin{figure}[H]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/device-utility/realfm-device-utility-16device.png}
   \caption{Average Device Utility Gained on CIFAR-10.}
   \label{fig:device-u-8-cifar} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/device-utility/realfm-device-utility-8device-mnist.png}
   \caption{Average Utility Gained on MNIST.}
   \label{fig:device-u-8-mnist}
\end{subfigure}
\caption{\textbf{Improved Device Utility for $8$ Devices on Real-World Data.}}
\label{fig:util-device-8}
\end{figure}

==> figures/old/mnist-accuracy-plots.tex <==
\begin{figure}[H]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-8device-mnist.png}
   \caption{Test Accuracy for 8 Devices.}
   \label{fig:mnist-acc-8} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/acc-figures/accuracy-comp-16device-mnist.png}
   \caption{Test Accuracy for 16 Devices.}
   \label{fig:mnist-acc-16}
\end{subfigure}
\caption{\textbf{Test Accuracy for Local versus Federated Training on MNIST.} As MNIST is an easier dataset to classify, both Local Training and FedAvg do great jobs at classifying digits. However, FedAvg does perform at a $99+$\% accuracy whereas Local Training sits around $97-98$\%. While this may seem to be a small gap, the utility gained by having a nearly perfect classification scheme is much greater than that having only $97$\%.}
\label{fig:mnist-acc}
\end{figure}

==> figures/old/mnist-server-16.tex <==
\begin{figure}[t]
\centering
   \begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-utility-16devices-mnist.png}
   \caption{Server Utility Comparison.}
   \label{fig:server-u-16-mnist} 
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-data-produced-16devices-mnist.png}
   \caption{Average Data Contribution Comparison.}
   \label{fig:server-g-16-mnist}
\end{subfigure}
\caption{\textbf{Improved Server Utility on MNIST.} Tasked with non-linear (and possibly non-uniform) payoff functions, \realfm achieves \textit{over 3 magnitudes} more server utility than a FL version of \citep{karimireddy2022mechanisms} (denoted as \textsf{Linear} \realfm). \realfm incentivizes devices to produce nearly $700$\% more data points (\ref{fig:server-g-16-mnist}) than on their own.}
\label{fig:mnist-server-16}
\end{figure}

==> figures/old/mnist-server-8.tex <==
\begin{figure}[H]
\centering
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-utility-8devices-mnist.png}
   \caption{Server Utility Comparison.}
   \label{fig:server-u-8-mnist}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
   \includegraphics[width=\textwidth]{figures/server-gain/realfm-server-data-produced-8devices-mnist.png}
   \caption{Average Data Contribution Comparison.}
   \label{fig:server-g-8-mnist}
\end{subfigure}
\caption{\textbf{Server Utility for $8$ Devices on MNIST.}}
\label{fig:mnist-server-8}
\end{figure}

==> figures/old/server-utility-comparison-16-old.tex <==
\begin{figure*}[!t]
\centering
%\hfill
   \begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-16devices.png}
   \label{fig:cifar-16-su} 
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-16devices-noniid0.6.png}
   \label{fig:cifar-16-0.6-su}
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-16devices-noniid0.3.png}
   \label{fig:cifar-16-0.3-su}
\end{subfigure}
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-16devices.png}
   \label{fig:mnist-16-su} 
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-16devices-noniid0.6.png}
   \label{fig:mnist-16-0.6-su}
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-16devices-noniid0.3.png}
   \label{fig:mnist-16-0.3-su}
\end{subfigure}
\vspace{-6mm}
\caption{\textbf{Improved Server Utility on CIFAR-10 \& MNIST.} \realfm increases server utility on CIFAR-10 (top row) and MNIST (bottom row) for $16$ devices compared to relevant baselines. \realfm achieves upwards of 2 magnitudes more utility than a FL version of \citet{karimireddy2022mechanisms}, denoted as \textsc{Linear} \realfm, across both uniform and various heterogeneous Dirichlet data distributions (left: uniform, center: D-0.6, right: D-0.3) as well as non-uniform costs (C) and accuracy payoff functions (P).}
\label{fig:server-utility-comparsion-16}
\end{figure*}

==> figures/old/server-utility-comparison-8-old.tex <==
\begin{figure*}[!h]
\centering
%\hfill
   \begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-8devices.png}
   \label{fig:cifar-8-su} 
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-8devices-noniid0.6.png}
   \label{fig:cifar-8-0.6-su}
\end{subfigure}
%\hfill
\begin{subfigure}[t]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-cifar10-8devices-noniid0.3.png}
   \label{fig:cifar-8-0.3-su}
\end{subfigure}
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-8devices.png}
   \label{fig:mnist-8-su} 
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-8devices-noniid0.6.png}
   \label{fig:mnist-8-0.6-su}
\end{subfigure}
%\hfill
\begin{subfigure}[b]{0.31\textwidth}
   \includegraphics[width=\textwidth]{figures/server-utility/realfm-average-server-utility-mnist-8devices-noniid0.3.png}
   \label{fig:mnist-8-0.3-su}
\end{subfigure}
\caption{\textbf{Improved Server Utility on CIFAR-10 \& MNIST.} \realfm increases server utility on CIFAR-10 (top row) and MNIST (bottom row) for $8$ devices compared to relevant baselines. \realfm achieves upwards of 2 magnitudes more utility than a FL version of \citet{karimireddy2022mechanisms}, denoted as \textsc{Linear} \realfm, across both uniform and various heterogeneous Dirichlet data distributions (left: uniform, center: D-0.6, right: D-0.3) as well as non-uniform costs (C) and accuracy payoff functions (P).}
\label{fig:server-utility-comparsion-8}
\end{figure*}

==> old/0-Abstract.tex <==
\begin{abstract}
Edge device participation in federating learning~(FL) has been typically studied under the lens of device-server communication (\textit{e.g.,} device dropout) and assumes an undying desire from edge devices to participate in FL.
As a result, current FL frameworks are flawed when implemented in real-world settings, with many encountering the free-rider problem.
In a step to push FL towards realistic settings, we propose \realfm: the first truly federated mechanism which (1) realistically models device utility, (2) incentivizes data contribution and device participation, and (3) provably removes the free-rider phenomena.
\realfm does not require data sharing and allows for a non-linear relationship between model accuracy and utility, which improves the utility gained by the server and participating devices compared to non-participating devices as well as devices participating in other FL mechanisms.
On real-world data, \realfm improves device and server utility, as well as data contribution, by up to $300$x and $7$x respectively compared to baselines.% mechanisms.


%a federated mechanism that realistically models device utility and incentivizes devices to participate in federated training, all while provably removing the free-rider phenomena.

%Unlike previous FL mechanisms, \realfm is the first to incentivize device participation and data contribution within a federated setting (no data sharing) while eliminating free-riding.

%Furthermore, by allowing a non-linear relationship between device accuracy and utility, \realfm improves the utility gained by the server and participating devices compared to non-participating devices as well as devices participating in other FL mechanisms.
%On real-world data, \realfm improves device and server utility, as well as data contribution, by up to 3 magnitudes and $7$x respectively compared to baseline mechanisms.
\end{abstract}

==> old/1-Introduction.tex <==
\vspace{-1em}
\section{Introduction}
\label{sec:intro}

% At this moment, there is a gap between the theoretical promise of FL and actual implementation of FL for various institutions. 
% We believe that tackling problems that arise in realistic settings of FL will further the adoption and usage of FL algorithms in the world. 
% Enabling implementation of FL will spur robust and well-trained models which perform well across a wide range of demographics, all done with enhanced privacy for all users.
%  Unfortunately, widespread implementation of FL frameworks in real-world settings has been impeded 

Federated Learning (FL) allows edge devices to collaboratively train a model under the orchestration of a central server (Centralized FL) or in a peer-to-peer manner (Decentralized FL). 
However, real-world implementation of FL frameworks remains stagnant due to a couple of key issues:

\textbf{(C1) Lack of Incentives}.
Current FL frameworks generally lack incentives to increase device participation.
This leads to training with fewer devices and data contributions, which subsequently reduces the model accuracy after federated training.
Incentivizing devices to participate in training and produce more data, especially from a central server's perspective, improves model performance (further detailed in Section \ref{sec:formulation}) which leads to greater benefit for the devices and server.

\textbf{(C2) Free-Rider Problem}.
Second, and more importantly, many FL frameworks run the risk of encountering the free-rider problem: devices do not contribute gradient updates or data yet reap the benefits of a well-trained collaborative model. 
Removing the free-rider effect in FL frameworks improves performance of trained models \citep{wang2022assessing, wang2023frad} and reduces security risks \citep{fraboni2021free, lin2019free, wang2022pass} for devices. 
By simultaneously encouraging device participation while alleviating the threat of free-riding in FL frameworks, we move a step closer towards widespread adoption of FL in the real world.

In this paper, we propose \realfm: a federated mechanism $\mathcal{M}$ (\textit{i.e.,} game) which a server in a FL setup implements to eliminate \textbf{(C1)} and \textbf{(C2)} when rational devices participate. 
\textit{The goal of \realfm is to design a reward protocol, with model-accuracy $a^r$ and monetary $R$ rewards, such that rational devices choose to participate and contribute more data.}
By increasing device participation and data contribution, a server trains a higher-performing model and subsequently attains greater \textbf{utility}.

Utility is the backbone of realistic FL settings. 
It describes the net benefit derived by devices and a server from training a model with accuracy $a$.
Higher model accuracy correlates to higher utility.
Every rational device $i$ aims to maximize its utility $u_i$.
In realistic settings, device utility $u_i$ is personal: each device relates accuracy to utility with a unique function $\phi_i$ and has unique training costs $c_i$.
Utility is the guiding factor in whether rational devices participate in a federated mechanism.
Devices will only participate if the utility $u_i^r$ gained within the mechanism, via its rewards $(a^r_i, R_i)$, outstrips the maximum utility gained from local training $u_i^o$.
We construct \realfm such that (i) server achieves increased utility and (ii) devices are guaranteed to receive rewards, through mechanism participation, which provide greater utility than local training $u_i^r \geq u_i^o$.
 




%The payoff function $\phi_i$, which quantifies the utility gained by device $i$ for a given model accuracy $a$, is heterogeneous (different devices can have different valuations of a model with accuracy $a$).
%Furthermore, each device $i$ has its own unique costs $c_i$.



% \textit{The goal of \realfm is to design a reward protocol, under unique device utilities, such that rational devices choose to participate and contribute more data.}




% Our mechanism, entitled \realfm, instructs the server on how to reward devices participating in federated training with model accuracy and possible monetary rewards.


% \fhc{In my mind, utility is an object in mechanism design. Through utility design, you hope that a solution that maximizes the utility gets you what you want. So, from that perspective, your utility should be designed to be positively correlated with server performance, device's incentive to participate and to share data (maybe there is more?). }

\textbf{Summary of Contributions}. 
%Overall, a truly federated mechanism which tackles both \textbf{(1)} and \textbf{(2)} and realistically models device utility is lacking in current literature.
%To fill this void, 
We propose \realfm, a truly federated (no data sharing) mechanism.
\realfm improves upon the previous federated mechanisms by,
\vspace{-0.5em}
\begin{enumerate}[leftmargin=*]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \item provably eliminating the free-rider effect by incentivizing devices to participate and contribute more data to the federated training process than they would on their own,
    \item properly modeling device utility, by allowing a non-linear relationship between accuracy and utility, thereby improving both server and device utility,
    \item producing state-of-the-art results towards improving utility (for both the server and devices), data contribution, and final model accuracy on real-world datasets.
\vspace{-1em}
\end{enumerate}

\input{figures/mechanism-diagram}


% properly models device utility, incentivizes device participation in a federated learning scheme, and 

% Our novel mechanism does not require data sharing and it provably eliminates the free-rider problem by incentivizing devices to maximize their gradient contributions.
% Furthermore, \realfm designs a more realistic utility function for all devices which more precisely measures how devices value a model's accuracy and subsequently fosters higher utility and increased gradient contributions.

%Within our research, we hope to incorporate a new utility function which better reflects how devices value a model’s accuracy.
%Second, this paper only covers the data-sharing regime. In FL, the common assumption is that data is not shared between devices or even between a device and the central server. 
%Within our research, we hope to provide a mechanism for data maximization in the true FL environment, where data is not shared.
%In our work, we tackle this free-rider problem by properly incentivizing devices to maximize the output of their gradient contributions.



==> old/2-RelatedWorks.tex <==
\section{Related Works}
\label{sec:related-works}

\textbf{Federated Mechanisms.}
Previous literature \citep{zhan2020learning, zhan2020big, zhan2021incentive, chen2020mechanism} have proposed mechanisms to solve \textbf{(C1)} and incentivize devices to participate in FL training.
However, these works fail to address \textbf{(C2)}, the free-rider problem, and have unrealistic device utilities.
In \citet{chen2020mechanism}, data sharing is allowed which is prohibitive in the FL setting, as one of the main motivations of FL is to train models in a privacy-preserving manner.
In \citet{zhan2020big, zhan2021incentive, zhan2020learning}, device utility incorporates a predetermined reward for participation in federated training, with no specification on how this amount is set by the server.
This is unrealistic, since rewards should be dynamic and depend upon the success (resulting model accuracy) of the federated training.
Setting too low of a reward impedes device participation while too high of a reward reduces the utility gained by the central server (and risks negative utility if performance lags total reward paid out).
%Setting too low of a reward impedes device participation which subsequently reduces the performance of a trained model.
%Setting too high of a reward reduces the utility gained by the central server, and possibly incurs negative utility, if the model performance after training is not good enough to outweigh the large reward paid out to each device.
Overall, being able to predict an optimal reward \textit{prior} to training is unrealistic.

The recent work by \citet{karimireddy2022mechanisms} is the first to simultaneously solve \textbf{(C1)} and \textbf{(C2)}.
They propose a mechanism which incentivize devices to both (i) participate in training and (ii) produce more data than on their own (data maximization).
By incentivizing devices to maximize production of local data, the free-rider effect is eliminated.
% Furthermore, incentivizing devices to produce data also results in a trained model which achieves greater performance, and utility, for both the central server and all devices (more training data usually corresponds with higher-performing models).
While this proposed mechanism is a great step forward for realistic mechanisms, pressing issues remain. 
First, \citet{karimireddy2022mechanisms} requires data sharing between devices and the central server.
This is acceptable if portions of local data is able to be shared (\textit{i.e.} no privacy risks exist for certain subsets of local data), yet it runs counter to the original draw of FL: a privacy-preserving training method which \textit{does not require} sharing personal data.
Second, device utility is designed in \citet{karimireddy2022mechanisms} such that \emph{the utility improves linearly with increasing accuracy}.
We find this unrealistic, as an increase in model accuracy from $49$\% to $50$\% should not hold the same utility as an increase from $98$\% to $99$\%. 

\textbf{Contract Theory and Federated Free Riding.}
Contract theory in FL aims to optimally determine the balance between device rewards and registration fees (cost of participation).
In contract mechanisms, devices can sign a contract from the server specifying a task, reward, and registration fee.
If agreed upon, the device signs and pays the registration fee.
Each device receives the reward if it completes the task and receives nothing if it fails.
Contract mechanisms have the ability to punish free riding in FL by creating negative incentive if a device does not perform a prescribed task (\textit{i.e.,} it will lose its registration fee).
\citet{kang2019incentive, liu2022contract, lim2021towards, wang2021federated, cong2020game, lim2020hierarchical} propose such contract-based FL frameworks.
While effective at improving model
generalization accuracy and utility \citep{liu2022contract, lim2020hierarchical}, 
these works focus on optimal design of rewards to devices.
Our mechanism does not require registration fees, which further boosts device participation, and utilizes an accuracy shaping method to provide rewards at the end of training in an optimal and more realistic approach. 
Furthermore, like \citet{karimireddy2022mechanisms}, our mechanism incentivizes increased contributions to federated training which is novel compared with the existing contract theory literature and mechanisms.




==> old/3-Formulation.tex <==
\section{Preliminaries}
\label{sec:formulation}

Data reigns supreme when it comes to machine learning (ML) model performance; model accuracy improves as the quantity of training data increases assuming consistency of data quality \citep{junque2013predictive,zhu2012we,tramer2020differentially}.
Empirically, one finds that accuracy of a model is both concave and non-decreasing with respect to the amount of data used to train it \citep{sun2017revisiting}. 
Training of a ML model generally adheres to the law of diminishing returns: improving model performance by training on more data is increasingly fruitless once the amount of training data is already large. 
Similar to \citet{karimireddy2022mechanisms}, we model accuracy in terms of $m$ data points, difficulty of learning task $k>0$, and optimal attainable accuracy $a_{opt} \in [0, 1)$,
\begin{align}
    \label{eq:gen-bound}
        a(m) &:= \max (\hat{a}(m), 0), \quad \hat{a}(m) := a_{opt} - \frac{\sqrt{2k(2 + \log (m/k))}+4}{\sqrt{m}}.
\end{align}
While we find empirically that $a(m)$ is both concave and non-decreasing with respect to the number of data points $m$, it is difficult to find a suitable function, such as $\hat{a}(m)$ in \Eqref{eq:gen-bound}, whose range is restricted to $[0,1)$. 
Therefore, we allow the accuracy function $a(m): \sZ^+_0 \rightarrow [0, a_{opt})$ to take the form shown in \Eqref{eq:gen-bound}.
The rationale behind this formulation is rooted in a generalization bound which can be found in Appendix \ref{app:acc-modeling}.
%This is a slight variation to the accuracy functions in \citep{zhan2020learning, karimireddy2022mechanisms}, yet it remains valid as the number of unique gradients matches the number of data samples $m$ in a given dataset $\gD$ ($g=|\gD|=m$).
\begin{assumption}
    \label{assum:a1}
    Accuracy functions $a(m): \sZ^+_0 \rightarrow [0,a_{opt})$ and $\hat{a}(m): \sZ^+ \rightarrow (-\infty ,a_{opt})$ are both continuous and non-decreasing. $a(m)$ has a root at 0: $a(0) = 0$ and $\hat{a}(m)$ is concave. 
\end{assumption} 
Assumption \ref{assum:a1} ensures that we model accuracy as we find it empirically: continuous, non-decreasing, and experiencing diminishing returns (concave) with respect to the number of data points $m$. 

In the foundational federated algorithm FedAvg \citep{mcmahan2017communication}, a server sends down a current iteration $t$ version of the parameters $\bm{w^t}$.
Devices perform $h$ local gradient updates (using their own data) on $\bm{w^t}$ before sending the result to a central server which aggregates all local updates together into $\bm{w^{t+1}}$.
This process is repeated until an optimum or a near optimum is reached.
Our paper follows this same FL setting, with $n$ devices collaboratively train the parameters $\bm{w}$ of a ML model.
Each device has its own local dataset $\gD_i$ (which can change in size) containing data independently chosen from a common distribution $\mathsf{D}$ (known as the IID setting).
Unlike FedAvg and many FL methods, we \textit{do not require} devices participate in training.
Instead, devices collaborate with a central server only when they deem it beneficial for their own utility (\textit{i.e.}, collaboration with the central server results in a model with higher accuracy or monetary rewards). 
In the FL setting, we redefine $m$ to become $m_i := |\gD_i|$ for a device $i$ and $m := \sum_j |\gD_j|$ for all participating devices.

%Just as in FedAvg, each device $i$ returns a model to the server which has been updated on-device with local data for $\tau$ units of time \fhc{How is $\tau$ used? Should it have a device index?}. 

%a subset of the $g_i$ unique gradients for $h$ steps.
%In the IID setting, this is equivalent to $h$ steps of local training on the subset of all $g$ unique gradients by the central server.

% {\textcolor{blue}{AKS: Provide some context as to why we need this assumption and that it's general enough.}}

% {\textcolor{blue}{AKS: Clarify here how to interpret this when FedAvg is under consideration, as it's model updates instead of gradients, and model updates are the sum of gradients at different model weights}}


% {\textcolor{blue}{AKS: SPK's paper also takes the IID setting, can we say something or have anything related to non-IID settings?}}

% {\textcolor{blue}{AKS: Notation wise, use bold face for vectors/matrices and normal text for scalars, improves readability considerably.}}




%Each device $i$ collects and stores data independently chosen from a common distribution $\mathsf{D}$ (known as the IID setting).
%This means that (i) the size of each device's local dataset $\gD_i$ is allowed to vary over the course of training and (ii) devices partake in an IID setting.
%Our federated setting involves $n$ devices training a ML model, having parameters $w_i$, with a local dataset $\gD_i$ for each device $i$. 
%It is not assumed that devices must interact or collaborate with a central server. 
%While not assumed, devices are \textit{still able} to collaborate with a central server if they deem it beneficial for their own utility (\textit{i.e.}, collaboration with the central server results in a model with higher accuracy or monetary rewards). 
%We assume that each device collects and stores data independently chosen from a common distribution $\mathsf{D}$ (this is known as the IID setting).
%This means that (i) the size of each device's local dataset $\gD_i$ is allowed to vary over the course of training and (ii) devices partake in an IID setting.


==> old/3-Preliminaries-Old.tex <==
\section{Problem Setting}
\label{sec:formulation}

Data reigns supreme when it comes to model performance; model accuracy improves as the quantity of training data increases assuming consistency of data quality \citep{junque2013predictive,zhu2012we,tramer2020differentially}.
Empirically, one finds that accuracy of a model is both concave and non-decreasing with respect to the amount of data used to train it \citep{sun2017revisiting}. 
Training of a machine learning (ML) model generally adheres to the law of diminishing returns: improving model performance by training on more data is increasingly fruitless once the amount of training data is already large. 

In our work, we look to precisely represent the relationship between accuracy and data.
Similar to \citet{karimireddy2022mechanisms}, we represent accuracy in terms of the number of data points $m$ and difficulty of learning task $k>0$.
A larger $k$ signifies a more difficult task, and $k$ remains constant for all devices.
One major novelty of our work, unlike, \citet{karimireddy2022mechanisms}, is that we also take into account differing data distributions.
Instead of assuming that all data is independently chosen from a common distribution (known as the IID setting), we generalize to the heterogeneous and non-IID setting.
This is important, as the distribution of data upon which a model is trained can dramatically affect the best accuracy $a_{opt}$ a model can attain.
Therefore, each device $i$ can have its own data distribution $\mathcal{D}_i$ with its subsequent optimal attainable accuracy $a_{opt}^i := a_{opt}(\mathcal{D}_i) \in [0, 1)$.
\fh{Here, $a_{opt}^i$ models the upper bound of accuracy when learning on a single device alone.
$k$ is reserved to represent task difficulty related to the collaborative distributed learning setting rather than the upper bound of learning on a single specific device.}
 \fhc{I think the problem here is why $k$ isn't already included in this $a_{opt}^i$.}

\textbf{Device Accuracy Representation}. Since accuracy depends upon the data distribution for each device, we represent accuracy differently for each device $i$,
\begin{align}
    \label{eq:gen-bound}
        \hat{a}_i(m) &:= a_{opt}^i - \frac{\sqrt{2k(2 + \log (m/k))}+4}{\sqrt{m}}, \\
        \label{eq:acc}
        a_i(m) &:= \max (\hat{a}_i(m), 0).
\end{align}
While we find empirically that $a_i(m)$ is both concave and non-decreasing with respect to the number of data points $m$, it is difficult to find a suitable function, such as $\hat{a}_i(m)$ in \Eqref{eq:gen-bound}, whose range is restricted to $[0,1)$. 
Therefore, we allow the accuracy function $a_i(m): \sZ^+_0 \rightarrow [0, a_{opt}^i)$ to take the form shown in \Eqref{eq:acc}.
The rationale behind this formulation is rooted in a generalization bound which can be found in Appendix \ref{app:acc-modeling}.
\begin{assumption}
    \label{assum:a1}
    Accuracy functions $a_i(m): \sZ^+_0 \rightarrow [0,a_{opt}^i)$ and $\hat{a}_i(m): \sZ^+ \rightarrow (-\infty ,a_{opt}^i)$ are continuous and non-decreasing. $a_i(m)$ has a root at 0: $a_i(0) = 0$, and $\hat{a}_i(m)$ is concave. 
\end{assumption} 
Assumption \ref{assum:a1} ensures that we capture the empirical relationship between data $m$ and ML model accuracy $a_i(m)$: $a_i(m)$ is continuous, non-decreasing, and experiencing diminishing returns (concave) with respect to $m$.

\fh{1. What is $a_{opt}^i$ and why it relates to }
% Assumption \ref{assum:a1} ensures that we represent the accuracy of a ML model, $a_i(m)$, as it is found empirically: continuous, non-decreasing, and experiencing diminishing returns (concave) with respect to the amount of training data $m$.

\fhc{Should we move assumption 1 outside of Preliminaries? I don't think this assumption is a preliminary. I think you don't need them until the theory section.}


\fhc{I am thinking, can we reverse the order of the paragraph of `Device Accuracy Representation' and `Assumption 1'? The narrative goes like: We allow pretty general and realistic relationship between accuracy and data, with mild assumptions. Put Assumption 1. Our mechanism design works with any accruacy-data relationship that satisfies Assumption 1. But for easy of demonstration, we will use this specific accuracy-data relationship function. Put the paragraph of `Device Accuracy Representation'.}

\textbf{Server Accuracy Representation}. The central server will also have its own accuracy function $a_C(m)$.
Since the central server aggregates device updates which stem from potentially heterogeneous data distributions, the optimal server accuracy is defined as the expectation of these unique accuracy functions,
\begin{align}
    \hat{a}_C(m) &:= \E_{i \in [n]} \left[ a_{opt}^i - \frac{\sqrt{2k(2 + \log (m/k))}+4}{\sqrt{m}}  \right], \nonumber \\
    \label{eq:server-acc}
    &= \bar{a}_{opt} -\frac{\sqrt{2k(2 + \log (m/k))}+4}{\sqrt{m}}, \\
    a_C(m) := &\max (\hat{a}_C(m), 0), \;\; \bar{a}_{opt} := \sum_{i=1}^n \frac{m_i}{\sum \bm{m}}  a_{opt}^i.
    \label{eq:server-acc-2}
\end{align}
As the expectation of all device accuracy functions, $a_C(m)$ and $\hat{a}_C(m)$ also follow Assumption \ref{assum:a1}.

%One can see that we define the server's optimal accuracy as the expectation of all of its participating devices' $\bar{a}_{opt} := \sum_{i=1}^n \frac{m_i}{\sum \bm{m}} a_{opt}^i$.

\textbf{Review of Federated Learning Paradigm}. In FedAvg \citep{mcmahan2017communication}, a server $C$ sends down a current iteration $t$ version of the parameters $\bm{w^t}$.
Devices perform $h$ local gradient updates (using their own data) on $\bm{w^t}$ before sending the result to a central server which aggregates all local updates together into $\bm{w^{t+1}}$.
This process is repeated until an optimum or a near optimum is reached.
Our paper follows this same FL setting with $n$ devices collaboratively training the parameters $\bm{w}$ of a ML model.
Each device has its own local dataset $\gD_i$ (which can change in size and distribution) which can differ device to device.
Unlike FedAvg and many FL methods, we \textit{do not require} devices participate in training.
Instead, devices collaborate with a central server only when they deem it beneficial for their own utility (\textit{i.e.}, collaboration with the central server results in a model with higher accuracy or monetary rewards). 
In the FL setting, we redefine $m$ to become $m_i := |\gD_i|$ for device $i$ and $m := \sum_j |\gD_j|$ for all participating devices.




==> old/4-Realistic-Utility.tex <==
\section{Realistic Device Utility}
\label{sec:dev-utility}

\realfm improves upon previous federated mechanisms, such as \citet{karimireddy2022mechanisms, zhan2021incentive, zhan2020big}, by modeling utility in a more realistic manner.
Specifically, we design a utility which: \textbf{(D1) Realistically Relates Accuracy to Utility} \textbf{(D2) Allows Non-Deterministic Rewards}.

To tackle \textbf{(D1)}, we propose utilizing an accuracy payoff function $\phi_i(a): [0,1) \rightarrow \sR_{\geq 0}$, which allows for a flexible definition of the benefit device $i$ receives from having a model with accuracy $a$. 
In \citet{karimireddy2022mechanisms}, it is assumed that $\phi_i$ is linear, $\phi_i(a) = a$, for all devices, which may not hold in many instances.
Non-linearity is necessary to precisely relate accuracy to utility, however, as accuracy improvement from 49\% to 50\% should be rewarded much differently than 98\% to 99\%.
Therefore, we generalize $\phi_i$ to become a convex and increasing function (which includes the linear case).
The convex and increasing requirements stems from the idea that increasing accuracy leads to increasing benefit for rational devices.
\begin{assumption}
    \label{assum:a2}
    Each device $i$'s accuracy payoff function $\phi_i(a(m)): [0, a_{opt}) \rightarrow \sR_{\geq 0} $ is continuous, non-decreasing, and has a root at 0: $\phi_i(0) = 0$. Furthermore, $\phi_i(a)$ is convex and strictly increasing with respect to $a$, while $\phi_i(a(m))$ is concave and strictly increasing $\forall m \text{ such that } \hat{a}(m) \geq 0$.
\end{assumption}
Many realistic choices for $\phi_i$ which satisfy Assumption \ref{assum:a2} exist.
One reasonable choice is $\phi_i(a) = \frac{1}{(1-a)^2} - 1$.
%When modeling $a(m)$ like in \Eqref{eq:gen-bound}, one reasonable choice for $\phi_i$ is $\phi_i(a) = \frac{1}{(1-a)^2} - 1$.
This choice of $\phi_i$ more precisely models how utility should grow as accuracy approaches 100\%, especially when compared to the linear relationship $\phi_i(a) = a$.

\subsection{Defining Server Utility}
\label{subsec:server-utility}

\textit{The overarching goal for a central server $C$ is to attain a high-performing ML model resulting from federated training.}
As discussed in Section \ref{sec:formulation}, ML model accuracy is assumed to improve as the total amount of data contributions $\bm{m}$ increases.
Therefore, server utility $u_C$ is a function of model accuracy which in turn is a function of data contributions,
\input{figures/marginal-cost-comparison}
\begin{equation}
    \label{eq:server-utility}
    u_C\left(\bm{m}\right) := p_m \cdot \phi_C\left(a\left(\sum \bm{m}\right)\right).
\end{equation}
The parameter $p_m \in (0, 1]$ denotes the central server's profit margin (percentage of utility kept by the central server).
Server utility in \Eqref{eq:server-utility} is maximized when model accuracy approaches 100\%, which in turn occurs when $\sum \bm{m} \rightarrow \infty$. 
The more data contributed by all devices $\bm{m}$ to the server, the better a ML model performs.
The better a ML model performs, the greater server utility becomes.
Thus, an optimal mechanism $\mathcal{M}$ from the server's standpoint \textit{would be one which incentivizes data contributions.}

Through the use of the profit margin $p_m$ in \Eqref{eq:server-utility}, we are able to tackle \textbf{(D2)} and allow for non-deterministic rewards.
Only a $p_m$ fraction of the total collected utility is kept by the server in \Eqref{eq:server-utility}.
The remaining $(1-p_m)$ utility can be distributed back to participating devices in any manner.
In Section \ref{subsec:rewards}, we detail how \realfm distributes the rewards proportionally to how much data each participating device contributes.


%The server utility in \Eqref{eq:server-utility} details that only a $p_m$ fraction of the total utility is kept by the server. \textit{Where does the remaining $(1-p_m)$ utility go?} This leftover utility forms the basis for our non-deterministic rewards.


% Using the definition of server utility in \Eqref{eq:server-utility} we also alleviate \textbf{(D2)}, the issue of providing predetermined rewards.\fh{how?} Once training is complete, and a final model accuracy is attained, the total server utility is computed using \Eqref{eq:server-utility}.  A fraction $p_m$ of the total utility is kept by the server, and the remaining $(1-p_m)$ utility is dispersed evenly amongst participating devices as a monetary reward. We detail this reward payout process in Section \ref{subsec:rewards}.

\subsection{Defining Local Device Utility}
\label{subsec:device-utility}
While increasing the amount of training data improves the performance of a model, it can be expensive for devices to collect more data.
Each device $i$ has its own fixed marginal cost $c_i > 0$, which represents the cost for collecting and computing an extra data point.
For example, the cost incurred for collecting $m$ data points would be $c_im$.
Overall, a device must weigh the cost incurred for collecting more data versus the benefits obtained from having a more accurate model.
We model this relationship through the use of a utility function $u_i$ for each device $i$.
Mathematically, the utility for each device $i$ is defined as,
\begin{equation}
\label{eq:utility}
    u_i(m) = \phi_i(a(m)) - c_im.
\end{equation}
The utility $u_i$ for each device $i$ is a function of data contribution: devices determine how many data points $m$ to collect in order to balance the benefit of model accuracy $\phi_i(a(m))$ versus the costs of data collection $-c_im$.

\begin{theorem}[Optimal Local Data Collection]
\label{thm:local-optimal}
    Consider device $i$ with marginal cost $c_i$, accuracy function $\hat{a}(m)$ satisfying Assumption \ref{assum:a1}, and accuracy payoff $\phi_i$ satisfying Assumption \ref{assum:a2}. Device $i$ collects an optimal amount of data $m_i^o$,
    \begin{equation}
    \label{eq:local-optimal}
        m_i^o = \begin{cases} 
      0 & \text{if } \max_{m_i \geq 0} u_i(m_i) \leq 0, \\
      m^*, \text{ such that } \phi_i'(\hat{a}(m^*))\cdot\hat{a}'(m^*) = c_i & \text{else.} 
   \end{cases}
    \end{equation}
\end{theorem}

Theorem \ref{thm:local-optimal} details how much data a device collects when \textit{training on its own and thereby not participating in a federated training scheme}.
Figure \ref{fig:utility-comparison} showcases utility peaks for both non-linear and linear accuracy payoff functions.
Figure \ref{fig:high-mc} shows that utility peaks at a negative value when marginal costs become too large.
In this case, as shown in Theorem \ref{thm:local-optimal}, devices do not contribute data.
We defer proof of Theorem \ref{thm:local-optimal} to Appendix \ref{app:proofs}.

%\begin{corollary}
%\label{cor:local-optimal}
%    Under uniform accuracy payoff functions $\phi_j(a(m)) = \phi_k(a(m)) \; \forall j,k$, two devices $j,k$ with respective marginal costs $c_j \leq c_k$ satisfy $u_j(m_j^o) \geq u_k(m_k^o)$ and $m_j^o \geq m_k^o$.
%\end{corollary}


==> old/5-Realistic-Mechanism.tex <==
\section{Realistic Federated Mechanisms}
\label{sec:fed-mech}

In the standard FL setting, devices are \textit{expected} to participate in training, i.e., send gradients or locally updated models to the central server.
However, this is not a realistic assumption in practice.
Many devices choose to participate in federated training only when it provides benefit, or utility, to them.
In the eyes of rational devices, they deserve adequate reward for shouldering computational burdens and providing valuable new gradient contributions.

To entice devices to participate in federated training, a central server must incentivize them.
Our paper covers two realistic rewards that a central server can provide: \textbf{(i)} model accuracy and \textbf{(ii)} monetary.
The interaction between the server and devices is formalized by a \textit{mechanism} $\mathcal{M}$.
When participating in the mechanism, a device $i$ performs federated training for a global model $\bm{w}$ on $m_i$ local data points in exchange for model accuracy $a^r(m_i) \in [0, a_{opt})$ and monetary $R(m_i) \in \sR_{\geq 0}$ rewards.
This exchange is defined as the following,
%If a device $i$ seeks to participate in federated training with the central server, it agrees to train the current global model $\bm{w^t}$ locally with its $m_i$ data points.
%After aggregating all device contributions, the central server assigns model accuracies or monetary rewards to each device based on their relative contribution.
%Mathematically, we formulate our proposed mechanism $\mathcal{M}(\bm{m})$ as following: for $n$ devices contributing $\bm{m}_{1:n}$ data points, they receive a model accuracy reward $a^r(m_i) \in [0, a_{opt})$ and monetary reward $R(m_i) \in \sR_{\geq 0}$ for each device $i$ from our mechanism,
\begin{equation}
    \mathcal{M}(m_1, \cdots, m_n) = \left( (a^r(m_1), R(m_1)), \cdots, (a^r(m_n), R(m_n)) \right).
\end{equation}

\input{RealFM-Algorithm}
\begin{definition}[Feasible Mechanism]
    \label{def:feasible}
    A feasible mechanism $\mathcal{M}$ (1) returns a bounded accuracy $0 \leq a^r(m_i) \leq a(\sum \bm{m})$ and non-negative reward $R(m_i) \geq 0$ to device $i$ and (2) is bounded in its provided utility $0 \leq u_i^r(\bm{m}) \leq u^r_{max}$.
\end{definition}

\begin{definition}[Individual Rationality]
    \label{def:ir}
    Let all devices contribute $\bm{m}$ data points and have $\bm{c}$ marginal costs. Mechanism $\mathcal{M}$ provides utility $u_i^r$ via model-accuracy $a^r(m_i)$ and monetary $R(m_i)$ rewards distributed to each device $i$. A mechanism satisfies individual rationality if for any device $i \in [n]$ (with maximum local utility $u_i^o$) and contribution $\bm{m}$,
    \begin{equation}
        \label{eq:ir}
        \phi_i \left( a^r(m_i) \right) + R(m_i) \geq \phi_i \left( a(m_i) \right) \equiv u_i^r \geq u_i^o.
    \end{equation}
\end{definition}
In order to incentivize devices to participate in a FL mechanism, it must (i) return a feasible utility $[\mathcal{M}^U(\cdot)]_i$ (fulfilling Definition \ref{def:feasible}) and (ii) provide utility that is greater than or equal to the utility gained by not participating and training alone (fulfilling Definition \ref{def:ir}).

\begin{theorem}[Existence of Pure Equilibrium]
\label{thm:pure-equ}
    Consider a feasible mechanism $\mathcal{M}$ returning utility $[\mathcal{M}^U(m_i; \bm{m}_{-i})]_i$ to device $i$ 
    ($[\mathcal{M}^U(0; \bm{m}_{-i})]_i = 0$).
    Participating device $i$'s utility is,
    %Define the utility of a participating device $i$ as, 
    \begin{equation}
        u_i^r(m_i; \bm{m}_{-i}) := [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i - c_im_i.
    \end{equation}
    If $u_i^r(m_i, \bm{m}_{-i})$, is quasi-concave for $m_i \geq m^u_i := \inf \{m_i \; | \; [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i > 0 \}$ and continuous in $\bm{m}_{-i}$, then a pure Nash equilibrium with $\bm{m^{eq}}$ data contributions exists,
    \begin{equation}
        \label{eq:pure-eq}
        u_i^r(\bm{m^{eq}}) = [\mathcal{M}^U(\bm{m^{eq}})]_i - c_i \bm{m^{eq}}_i \geq [\mathcal{M}^U(m_i; \bm{m^{eq}}_{-i})]_i - c_i m_i  \; \forall m_i \geq 0.
    \end{equation}
\end{theorem}
The proof of Theorem \ref{thm:pure-equ} is found in Appendix \ref{app:proofs}.
Our new proof amends and simplifies that of \citet{karimireddy2022mechanisms}, as we show $u_i^r$ only needs to be quasi-concave in $m_i$.

%Our proof of existence of a pure equilibrium for $\mathcal{M}$ follows from \citet{karimireddy2022mechanisms}, however we amend its requirements of $u_i^r$ (namely that it must be quasi-concave in $m_i$).
%This leads to a new proof.

\subsection{Defining Mechanism Rewards}
\label{subsec:rewards}
While the mechanism in \citet{karimireddy2022mechanisms} was the first federated mechanism proposed to maximize data collection, it required data sharing and lacked realistic assumptions on device utility.
We design a realistic and truly federated mechanism which incentivizes device participation and data contribution by returning \textbf{(i)} monetary rewards to devices when desirable and \textbf{(ii)} improved accuracy, via accuracy-shaping, under non-linear and non-uniform accuracy payoff functions $\phi_i$.

\textbf{Monetary Rewards}. 
As mentioned above in Section \ref{sec:fed-mech}, the federated mechanism $\mathcal{M}$ is posted by the central server.
The profit margin $p_m$ of the server is fixed and known by all devices when $\mathcal{M}$ is issued.
However, the accuracy payoff function for the central server $\phi_C$ is not known by the devices.

Section \ref{subsec:server-utility} details how the server maintains a $p_m$ fraction of utility it receives, as shown in \Eqref{eq:server-utility}, while distributing the remaining $(1-p_m)$ utility amongst participating devices as a monetary reward.
The reward is dispersed as a marginal monetary reward $r(\bm{m})$ per contributed data point,
\begin{equation}
    \label{eq:server-reward}
    %r(\bm{m}) := (1-p_m) \cdot \frac{\phi_C\left(a\left(\sum \bm{m}\right)\right)}{\sum \bm{m}}.
    r(\bm{m}) := (1-p_m) \cdot \phi_C\left(a\left(\sum \bm{m}\right)\right) / \sum \bm{m}.
\end{equation}
The marginal monetary reward $r(\bm{m})$ is dynamic and depends upon the total amount of data contributions from devices during federated training.
Therefore, $r(\bm{m})$ is unknown by devices when $\mathcal{M}$ is issued.
However, the server computes and provides the monetary rewards once training is complete.

\textbf{Accuracy Shaping}.
Accuracy shaping, the heart of any great federated mechanism, is responsible for incentivizing devices to collect more data than their local optimal amount $m_i^o$.
The idea behind accuracy shaping is to incentivize device $i$ to produce more data $m_i^* \geq m_i^o$ by providing it a boosted model accuracy whose utility outstrips the marginal cost of collecting more data $-c_i\left(m_i^* - m_i^o\right)$.

Our mechanism is related to \citet{karimireddy2022mechanisms} in that it also performs accuracy shaping, albeit in a more difficult setting.
Accuracy shaping with non-linear accuracy payoffs $\phi$ is far more difficult than with linear ones (\citet{karimireddy2022mechanisms} assumes a linear $\phi$).
To overcome the issues with non-linear $\phi$'s, we carefully construct an accuracy-shaping function $\gamma_i(m)$ for each device $i$.

\begin{theorem}[Accuracy Shaping Guarantees]
\label{thm:acc-shaping}
Consider a device $i$ with marginal cost $c_i$ and accuracy payoff function $\phi_i$ satisfying Assumption \ref{assum:a2}. Denote device $i$'s optimal local data contribution as $m_i^o$ and its subsequent accuracy $\bar{a} = a(m_i^o)$. 
Define the derivative of $\phi_i(a)$ with respect to $a$ as $\phi_i'(a)$.
For any $\epsilon \rightarrow 0^+$ and marginal server reward $r(\bm{m}) \geq 0$, device $i$ has the following accuracy-shaping function $\gamma_i(m)$ for $m \geq m_i^o$,
\begin{align}
\label{eq:gamma}
    \gamma_i := \begin{cases} \frac{-\phi_i'(\bar{a}) + \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a})(c_i - r(\bm{m}) + \epsilon) (m-m_i^o)}}{\phi_i''(\bar{a})} & \text{if } \phi_i''(\bar{a}) > 0\\
    \frac{(c_i - r(\bm{m}) + \epsilon)(m-m_i^o)}{\phi_i'(\bar{a})} & \text{if } \phi_i''(\bar{a}) = 0
    \end{cases}
\end{align}
Given the defined $\gamma_i(m)$, the following inequality is satisfied for $m \in [m_i^o, m_i^*]$,
\begin{equation}
\label{eq:gamma-satisfy}
\phi_i(a(m_i^o) + \gamma_i(m)) - \phi_i(a(m_i^o)) > (c_i - r(\bm{m}))(m - m_i^o).
\end{equation}
The new optimal contribution is $m_i^* := \{ m \geq m_i^o \; | \; a(m + \sum_{j \neq i} m_j)  =  a(m_i^o) + \gamma_i(m)\}$.
Accuracy shaping improves device $i$'s data contribution $m_i^* \geq m_i^o$ for any contribution $\bm{m}_{-i}$.
%Given all other device data contributions $\bm{m}_{-i}$, accuracy shaping improves device utility and results in a new optimal contribution $m_i^* \geq m_i^o$.
\end{theorem}
Theorem \ref{thm:acc-shaping}, whose full proof is found in Appendix \ref{app:proofs}, details the limits of accuracy shaping such that any mechanism can remain feasible.
To remain feasible, the central server cannot provide provide an accuracy beyond the sum of the total contributions $a(\sum \bm{m})$.
Devices which participate in $\mathcal{M}$ must share $c_i, \phi_i$ with the central server while the central server must provide $p_m$ when posting $\mathcal{M}$.
\begin{remark}
    For a linear accuracy payoff, $\phi_i(a) = wa$ for $w>0$, and thus $\phi_i''(a) = 0 \; \forall a$, \Eqref{eq:gamma} relays $\gamma_i = \frac{(c_i - r(\bm{m}) + \epsilon)(m - m_i^o)}{w}$. 
    We recover the accuracy-shaping function of Equation (13) in \citet{karimireddy2022mechanisms} with their no-reward $r(\bm{m})=0$ and $w=1$ linear setting.
    Thus, our accuracy-shaping function generalizes the one in \citet{karimireddy2022mechanisms}.
\end{remark}

\subsection{\realfm: a Realistic Federated Mechanism}

Pseudo-code for our mechanism, \realfm, is detailed in Algorithm \ref{alg:realfm}.
We begin by first defining the \textit{utility} $[\mathcal{M}^U(\bm{m})]_i$ that our mechanism returns to each device $i$,
\begin{align}
    \label{eq:mech-utility}
    &[\mathcal{M}^U(\bm{m})]_{i} = \begin{cases}
         \phi_i \big( a(m_i) \big) & \text{if } m_i \leq m_i^o\\
         \phi_i \big( a(m_i^o) + \gamma_i(m_i) \big) + r(\bm{m})(m_i - m_i^o) & \text{if } m_i \in [m_i^o, m_i^{*}] \\
          \phi_i \big( a(\sum \bm{m}) \big) + r(\bm{m})(m_i - m_i^{*}) & \text{if } m_i \geq m_i^{*}.
    \end{cases}
\end{align}
Now we mathematically formulate how $\mathcal{M}$ distributes model-accuracy and monetary rewards to each device participating in $\mathcal{M}$ given a collective data contribution $\bm{m}$,
\begin{align}
    \label{eq:mech}
    &\bigg( a^r(m_i), R(m_i) \bigg) = \begin{cases}
        \bigg( a(m_i), \; 0 \bigg) & \text{if } m_i \leq m_i^o\\
        \bigg( a\big(m_i^o\big) + \gamma_i(m_i), \; r(\bm{m})(m_i - m_i^o) \bigg) & \text{if } m_i \in [m_i^o, m_i^*] \\
         \bigg( a(\sum \bm{m}), \; r(\bm{m})(m_i - m_i^*) \bigg) & \text{if } m_i \geq m_i^*.
    \end{cases}
\end{align}

\begin{theorem}[Existence of Equilibrium with Increased Data Contribution]
\label{thm:main}
    Our realistic federated mechanism $\mathcal{M}$, defined in \Eqref{eq:mech}, performs accuracy-shaping with $\gamma_i$ defined in Theorem \ref{thm:acc-shaping} for each device $i \in [n]$ and some small $\epsilon \rightarrow 0^+$. 
    As such, $\mathcal{M}$ is Individually Rational (IR) and has a unique Nash equilibrium at which device $i$ will contribute $m_i^* \geq m_i^o$ updates, thereby eliminating the free-rider phenomena.
    Furthermore, since $\mathcal{M}$ is IR, devices are incentivized to participate as they gain equal to or more utility than by not participating.
\end{theorem}

\begin{corollary}
    When accuracy payoffs are linear for a device $i$, $\mathcal{M}$ defined in \Eqref{eq:mech} is contribution-maximizing. The proof follows from Theorem 4.2 in \citet{karimireddy2022mechanisms}.
\end{corollary}

Our usage of a non-linear accuracy payoff function $\phi_i$ promotes increased data production compared to a linear payoff (see Section \ref{sec:experiments}).
However, proof of data maximization for non-linear payoffs is not possible as one cannot perfectly bound the composition function $\phi(a + \gamma(m))$ as you can with the linear payoff $a + \gamma(m)$.
Our accuracy-shaping function is still data maximizing when linear.

\textbf{Honest Devices.} Our setting assumes honest devices. They only store the rewarded model returned by the server after training. 
In the case that devices are dishonest, slight alterations to the federated training scheme can be made.
Namely, schemes that train on varying-sized models such as \citep{diao2020heterofl, li2019fedmd, hu2021mhat, arivazhagan2019federated} can be implemented (where model sizes correspond to the amount of data contributed) to alleviate honesty issues.


% Due to the usage of a non-linear payoff function $\phi_i$, it is no longer to provable that $\mathcal{M}$ is data-maximizing
% [add a remark about the non-linear payoff contribution maximization]


==> old/6-Experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}
To test the efficacy of \realfm, we analyze how well it performs at \textbf{(i)} improving utility for the central server and devices, and \textbf{(ii)} increasing the amount of data contributions to the federated training process on image classification experiments.
We use CIFAR-10 \citep{krizhevsky2009learning} and MNIST \citep{deng2012mnist} as our real-world datasets.

\textbf{Experimental Baselines.} Few FL mechanisms eliminate the free-rider effect, with none doing so without sharing data, in the non-convex setting.
Therefore, we adapt the mechanism proposed in \citep{karimireddy2022mechanisms} as the baseline to compare against (we denote this adaptation as \textsf{Linear} \realfm).
We also compare \realfm to a local training baseline where
we measure the average device utility attained by devices if they did not participate in the mechanism.
Server utility is inferred in this instance by using the average accuracy of locally trained models.

\textbf{Testing Scenarios.} We denote (LP) as linear payoff and (NLP) as non-linear payoff.
We test \realfm under uniform (U-NLP) as well as non-uniform costs (NU-C) and payoffs \& costs (NU-PC).
Since \textsf{Linear} \realfm does not use a payoff function, we only test it under uniform (U-LP) and non-uniform costs (NU-C).
Finally, for local training, the non-uniform results are nearly identical to their uniform counterparts, so we remove them to save space.
\input{figures/cifar-server-16}

\textbf{Experimental Setup.}
Within our experiments, both $8$ and $16$ devices train a ResNet18 and a small convolutional neural network for CIFAR-10 and MNIST respectively.
As detailed in Appendix \ref{app:exp}, we carefully select and tune $a(m)$ to match the empirical training results on both datasets as closely as possible.
Once tuned, we select a marginal cost $c_e$ such that, by \Eqref{eq:local-optimal}, the local optimal data contribution is $3,000$ and $5,500$ ($3,500$ and $7,000$) for each of the $8$ and $16$ devices respectively on CIFAR-10 (MNIST).
When performing uniform cost experiments, each device uses $c_e$ as its marginal cost (and thus each device has the same amount of data).
For non-uniform cost experiments, $c_e$ is the mean of a Gaussian distribution from which the marginal costs are sampled.
Our uniform payoff function is $\phi_i(a) = \frac{1}{(1-a)^2} - 1$ for each device $i$.
For non-uniform payoff experiments, we set $\phi_i(a) = z_i(\frac{1}{(1-a)^2} - 1)$ where $z_i$ is uniformly sampled within $[0.9, 1.1]$.
A list of hyper-parameters, additional experimental details, and $8$ devices results are found in Appendix \ref{app:exp}.


\textbf{\realfm Dramatically Improves Server Utility.}
\realfm is powered by the incentives provided by its accuracy-shaping function. 
By Theorem \ref{thm:acc-shaping}, devices provably contribute more data when accuracy-shaping occurs.
As the total amount of data $m$ grows due to the incentives of accuracy shaping, a higher-performing model is trained by the server.
A higher-performing model results in higher utility for the server (\Eqref{eq:server-utility}).
This is backed up empirically, as Figures \ref{fig:server-u-16} and \ref{fig:server-u-16-mnist} showcase upwards of \textit{3 magnitudes greater utility} compared to state-of-the-art FL mechanisms.

\textbf{\realfm Incentivizes Devices to More Actively Contribute to Federated Training.}
Figures \ref{fig:server-g-16} and \ref{fig:server-g-16-mnist} showcase the power of \realfm, via its accuracy-shaping function, to incentivizes devices to contribute more data points.
Through its construction, \realfm's accuracy-shaping function incentivizes devices to contribute more data than they would locally in exchange for greater utility.
This is important for two reasons. First, incentivizing devices to contribute more than local training proves that the free-rider effect is not taking place.
Second, higher data contribution lead to better-performing models and higher accuracies.
This improves the utility for all participants.
Overall, \realfm is superior at incentivizing contributions compared to state-of-the-art FL mechanisms.

\textbf{\realfm Increases Device Utility.}
As shown in Figure \ref{fig:util-device-16}, devices participating in \realfm also boost their utility.
The improvement stems from (i) effective accuracy-shaping by \realfm and (ii) the use of non-linear payoff functions $\phi$, which more precisely map the benefit derived from an increase in model accuracy.
\realfm's accuracy-shaping function is defined (Theorem \ref{thm:acc-shaping}) to improve device utility if devices contribute more data than they would locally.
Incorporating $\phi$ into device utility makes it more realistic and spurs increased data contribution.
With utilities that grow increasingly great with improved accuracy, devices are incentivized to contribute more data in order to chase higher model accuracy and subsequent utility.

\input{figures/mnist-server-16}
\input{figures/device-utility-16}

==> old/7-Conclusion.tex <==
\vspace{-1em}
\section{Conclusion}
\label{sec:conclusion}
Without proper incentives, modern FL frameworks fail to attract devices to participate.
Furthermore, current FL mechanisms which incorporate incentives fall victim to the free-rider problem.
\realfm is the first FL mechanism which boosts device participation and data contribution all while eliminating the free-rider phenomena without requiring data to be shared.
Device and server utility is greatly improved in \realfm by the construction of a novel and realistic utility function which more precisely models the relationship between accuracy and utility.
Empirically we found that \realfm's realistic device utility and effective incentive structure, through the use of a novel accuracy-shaping function, resulted in higher-performing models during federated training.
As a result, \realfm provides higher utilities to the server and participating devices compared to its peer FL mechanisms.

==> old/9-Notes.tex <==
\newpage
\section{Ideas}



=================================
\textbf{Update Maximizing.} 
By virtue of our mechanism $\mathcal{M}$ utilizing the accuracy-shaping function $\gamma_i$ as prescribed in Theorem \ref{thm:acc-shaping}, each device $i$ will contribute $g_i^* \geq g_i^o$ updates as is proven in Theorem \ref{thm:acc-shaping}.
Below, we show that $\mathcal{M}$ is update-maximizing, \textit{i.e.} for any other other mechanism $\mathcal{\tilde{M}}$,
\begin{equation}
    g_i^* \geq \argmax_{g_i} \;[\mathcal{\tilde{M}}^U(g_i; \bm{g}_{-i})]_i - c_i g_i = \tilde{g}_i^*.
\end{equation}
To prove this, let's assume that \textit{there is} such a mechanism $\mathcal{\tilde{M}}$ such that $\tilde{g}_i^* > g_i^*$.
This implies,
\begin{equation}
    \tilde{u}_i'(g_i; \bm{g}_{-i}) = \frac{\partial [\mathcal{\tilde{M}}^U(g_i; \bm{g}_{-i})]_i}{\partial g_i} - c_i > 0,
\end{equation}
for all $g_i < \tilde{g}_i^*$.
Since $\tilde{g}_i^* > g_i^*$, then
$\tilde{u}_i'(g_i; \bm{g}_{-i})$ cannot equal zero for all $g_i < \tilde{g}_i^*$ as well.
This means that $\frac{\partial [\mathcal{\tilde{M}}^U(g_i; \bm{g}_{-i})]_i}{\partial g_i} > c_i$ for $g_i < \tilde{g}_i^*$.
As $\mathcal{\tilde{M}}$ must be individually rational (IR),
\begin{equation}
    [\mathcal{\tilde{M}}^U(g_i^o; \bm{g}_{-i})]_i \geq a(g_i^o) = [\mathcal{M}^U(g_i^o; \bm{g}_{-i})]_i.
\end{equation}
Therefore, 



Furthermore, this means that for all $g_i \in [g_i^o, g_i^*]$,
\begin{equation}
    \frac{\partial [\mathcal{\tilde{M}}^U(g_i; \bm{g}_{-i})]_i}{\partial g_i} > \frac{\partial [\mathcal{M}^U(g_i; \bm{g}_{-i})]_i}{\partial g_i}.
\end{equation}




[think about making mechanism strictly quasi-concave (always increasing)]

idea: if strictly quasi-concave, then can do  $> c_i*(b-g_i^o)$ and show we have that tight already
=================================

WEIGHT THE FED AVERAGING BY HOW MANY UPDATES EACH DEVICE CAN SEND (which is what normally happens)

\textbf{True Federated Mechanism}

\begin{enumerate}
    \item We model accuracy as a function of the number of batches of gradients (updates) available to the central server 
\end{enumerate}
In this manner, devices will want to collect more data since they will have more updates to provide to the central host.

\textit{Questions/Comments}

\begin{itemize}
    \item Requires assuming a fixed batch size $M$?
    \item Devices would have to send multiple local updates. Host could either (a) set a time limit on how long devices have to compute as many updates as possible (this does give advantage to fast workers, this is removed if all devices assumed to be equally fast) or (b) 
    \item Might need to perform ablations to showcase that more batches of gradients does indeed lead to higher accuracy. This is important to ensure concavity of accuracy function with respect to the number of batches of data.
\end{itemize}


%The federated process is summarized by the following steps:
%\begin{enumerate}[leftmargin=*]
%    \itemsep0em 
%    \item Central server issues a mechanism $\mathcal{M}$ within which devices can partake in federated training.
%\end{enumerate}
%\textbf{For Devices Partaking in $\mathcal{M}$ ($t = 1, \ldots, T$ iterations of federated training):}
%\begin{enumerate}[leftmargin=*]
%    \itemsep1pt
%    \setcounter{enumi}{1}
%    \item Device $i$ contributes $m_i^t$ unique --- given global model $\bm{w^t}$ within a set time-frame $\tau$ and sends them to the central server.
%    \item The central server aggregates all updates, applies the aggregated update to the global model $\bm{w^{t+1}}$, and sends the resulting global model back to each device.
%    \item After $T$ iterations, the central server returns a trained model to each device with an accuracy and possible monetary reward prescribed by $\mathcal{M}\left(\frac{1}{T}\sum_{t=1}^T m_1^t, \ldots, \frac{1}{T}\sum_{t=1}^T m_n^t\right)$.
%\end{enumerate}

==> old/RealFM-Algorithm.tex <==
\begin{algorithm}[!htbp]
\DontPrintSemicolon
  \KwInput{Data contributions $\bm{m}$, marginal costs $\bm{c}$, payoff functions $\bm{\phi}$, profit margin $p_m$, $h$ local steps, $T$ total iterations, total local epochs $E$, initial model parameters $\bm{w^1}$, loss $\ell$, step-size $\eta$, accuracy-shaping function $\gamma_i(m)$, and accuracy function $a(m)$.}
  \KwOutput{Model with accuracy $a^r(m_i)$ and monetary reward $R(m_i)$.}
  $s_i \leftarrow m_i / \sum_{j=1}^{n} m_j$ \tcp*{compute self-weight for federated averaging}
  \For{$t = 1, \ldots, T$}{
    Server distributes $\bm{w^t}$ to all devices\;
    \For{$h$ local steps, each device $i$ \textbf{in parallel}}{
    $\bm{w_i^{t+1}} \leftarrow$ ClientUpdate($i, \bm{w^t}$)
    }
    $\bm{w^{t+1}} \leftarrow \sum_j s_j \bm{w_i^{t+1}}$
    }
    $r(\bm{m}) \leftarrow (1-p_m)\frac{\phi_C\left(a\left(\sum_j m_j\right)\right)}{\sum_j m_j}$ \tcp*{compute monetary reward}
    \For{$i = 1$ to $n$}{
    Compute $m_i^o$ and $m_i^*$ using $c_i, \phi_i$, and $\gamma_i(m_i)$\;
    Return $(a^r(m_i), R(m_i))$ to device $i$ using $m_i, m_i^o, m_i^*, a(m), \gamma_i(m_i), \phi_i, r(\bm{m})$ in Eq. \ref{eq:mech}
    }
    \vspace{0.25\baselineskip}
    ClientUpdate($i, \bm{w}$):\;
    $\mathcal{B} \leftarrow$ batch $m_i$ data points\;
     \For{each epoch $e = 1, \ldots, E$}{
     \For{batch $b \in \mathcal{B}$}{
     $\bm{w} \leftarrow \bm{w} - \eta \nabla \ell(\bm{w}; b)$
    }
    }
\caption{\realfm: A Realistic Federated Mechanism}
\label{alg:realfm}
\end{algorithm}


==> old/a0-notation.tex <==
\section{Notation \& Related Work}
\label{app:notation}
\input{notation-table}

\textbf{Federated Mechanisms (Continued).}
As detailed in Section \ref{sec:related-works}, there is a wide swath of mechanisms proposed for FL.
The works \citep{zhan2021incentive, tu2022incentive, zeng2021comprehensive, ali2023systematic} survey the different methods of incentives present in FL literature.
The goal of the presented methods are solely to increase device participation within FL frameworks.
The issues of free riding and increased data or gradient contribution are not covered.
\citep{sim2020collaborative, xu2021gradient} design model rewards to meet fairness or accuracy objectives. 
In these works, as detailed below, devices receive models proportionate to the amount of data they contribute but are not incentivized to contribute more data.
Our work seeks to incentivize devices to contribute more during training.

\textbf{Collaborative Fairness and Federated Shapley Value.}
Collaborative fairness in FL \citep{lyu2020collaborative, lyu2020towards, xu2020reputation, sim2020collaborative} is closely related to our paper. 
The works \citet{lyu2020collaborative, lyu2020towards, xu2020reputation, sim2020collaborative} seek to fairly allocate models with varying performance depending upon how much devices contribute to training in FL settings. 
This is accomplished by determining a "reputation" (a measure of device contributions) for each device, using a hyperbolic sine function, to enforce devices converge to different models relative to their amount of contributions during FL training.
Thus, devices who contribute more receive a higher-performing model than those who do not contribute much.
There are a few key differences between this line of work and our own, namely: \textbf{(1)} Our mechanism incentivizes devices to both participate in training and increase their amount of contributions. 
There are no such incentives in collaborative fairness.
\textbf{(2)} We model device and server utility. Unlike collaborative fairness, we do not assume that devices will always participate in FL training.
\textbf{(3)} Our mechanism design \textit{provably} eliminates the free-rider phenomena unlike collaborative fairness, since devices who try to free-ride receive the same model performance as they would on their own (Equations \ref{eq:mech-utility} and \ref{eq:mech}).
\textbf{(4)} No monetary rewards are received by devices in current collaborative fairness methods.

While the overarching goal of our work is to incentivize and increase device participation, through mechanism design, within FL, important future research directions remain.
Federated Shapley Value, first proposed in \citet{wang2020principled}, allows for estimation of the Shapley Value in a FL setting.
This is crucial to appraise the data coming from each device and pave the way for rewarding devices with important data during the training process.
Data is not equally valuable in real-world settings, and relaxing the assumption of equally valued data within our paper is important future work.
We aim to use \citet{wang2020principled} to tackle the problem of data heterogeneity.

\input{figures/utility-comparison}

==> old/a1-proofs.tex <==
\section{Proof of Theorems}
\label{app:proofs}


\begin{reptheorem}{thm:local-optimal}
    Consider a device $i$ with marginal cost per data point $c_i$, accuracy function $\hat{a}(m)$ satisfying Assumption \ref{assum:a1}, and accuracy payoff $\phi_i$ satisfying Assumption \ref{assum:a2}. This device will collect the following optimal amount of data $m_i^o$:
    \begin{equation}
        m_i^o = \begin{cases} 
      0 & \text{if } \max_{m_i \geq 0} u_i(m_i) \leq 0, \\
      m^*, \text{ such that } \phi_i'(\hat{a}(m^*))\cdot\hat{a}'(m^*) = c_i & \text{else.} 
   \end{cases}
    \end{equation}
\end{reptheorem}
\begin{proof}
    Let $m_0 := \sup \{ m \; | \; \hat{a}(m) = 0 \}$ (the point where $a(m)$ begins to increase from 0 and become equivalent to $\hat{a}(m)$). Thus, $\forall m_i > m_0, a(m_i) = \hat{a}(m_i) > 0$. 
    Also, given Assumptions \ref{assum:a1} and \ref{assum:a2} and \Eqref{eq:utility},  $u_i(0) = 0$. 
    The derivative of \Eqref{eq:utility} for device $i$ is,
    \begin{equation}
    \label{eq:utility-deriv-1}
        u'_i(m_i) = \phi_i'(a(m_i))\cdot a'(m_i) - c_i.
    \end{equation}

    \textbf{Case 1: $\max_{m_i \geq 0} u_i(m_i) \leq 0$}. 
    
    Each device $i$ starts with a utility of 0 since by Assumptions \ref{assum:a1} and \ref{assum:a2} $u_i(0) = 0$. Since $\max_{m_i \geq 0} u_i(m_i) \leq 0$, there is no utility gained by device $i$ to contribute more data. 
    Therefore, the optimal amount of contributions remains at zero: $m_i^* = 0$.

    \textbf{Case 2: $\max_{m_i \geq 0} u_i(m_i) > 0$}.
    
    \textit{Sub-Case 1: $0 \leq m_i \leq m_0$}. By definition of $m_0$, $a(m_i) = 0 \; \forall m_i \in [0, m_0]$. Therefore, from \Eqref{eq:utility} and Assumptions \ref{assum:a1} and \ref{assum:a2}, $u_i(m_i) = - c_i m_i < 0 \; \forall m_i \in (0, m_0]$. Since $u_i(0) = 0$ and $u_i(m_i) < 0$ for $m_i > 0$, device $i$ will not collect any contribution: $m_i^* = 0$.
    
    \textit{Sub-Case 2: $m_i > m_0$}. Since $\forall m_i > m_0, a(m_i) = \hat{a}(m_i) > 0$, \Eqref{eq:utility-deriv-1} becomes,
    \begin{equation}
    \label{eq:utility-deriv-2}
        u'_i(m_i) = \phi_i'(\hat{a}(m_i))\cdot \hat{a}'(m_i) - c_i.
    \end{equation}
    We begin by showing that $\phi_i(\hat{a}(m_i))$ is bounded.
    By Assumption \ref{assum:a1}, $\hat{a}(m_i) < a_{opt} < 1 \; \forall m_i$. 
    Thus, $\phi_i(\hat{a}(m_i)) < \phi_i(a_{opt}) < \infty \; \forall m_i$ since $\hat{a}(m_i)$ and $\phi_i$ are non-decreasing and continuous by Assumptions \ref{assum:a1} and \ref{assum:a2}.
    Due to $\phi_i(\hat{a}(m_i))$ being concave, non-decreasing, and bounded (by Assumption \ref{assum:a2}), we have from \Eqref{eq:utility-deriv-2} that the limit of its derivative, 
    \begin{equation}
        \lim_{m_i \rightarrow \infty} \phi_i'(\hat{a}(m_i))\cdot \hat{a}'(m_i) = 0 \implies \lim_{m_i \rightarrow \infty} u_i'(m_i) = -c_i < 0.
    \end{equation}
    Since $\phi_i(\hat{a}(m_i))$ is concave and non-decreasing, its gradient $\phi_i'(\hat{a}(m_i))\cdot \hat{a}'(m_i)$ is maximized when $m_i = m_0$ and is non-increasing afterwards.
    Using the maximal derivative location $m_i = m_0$ in union with Case 2 ($\max_{m_i \geq 0} u_i(m_i) > 0$) and Sub-Case 2 ($u_i(m) \leq 0 \; \forall m \in [0, m_0]$) yields $u_i'(m_0) > 0$ (the derivative must be positive in order to increase utility above 0).

    Now that $u_i'(m_0) > 0$, $\lim_{m_i \rightarrow \infty} u_i'(m_i) < 0$, and $\phi_i'(\hat{a}(m_i))\cdot \hat{a}'(m_i)$ is non-increasing, there must exist a maximum $m_i = m^*$ such that $\phi_i'(\hat{a}(m^*))\cdot\hat{a}'(m^*) = c_i$.
\end{proof}

\begin{corollary}
\label{cor:local-optimal}
Under uniform payoff functions $\phi_i(a(m)) = \phi(a(m)) \; \forall i$, two devices $j,k$ with respective marginal costs $c_j \leq c_k$ satisfy $u_j(m_j^o) \geq u_k(m_k^*)$ and $m_j^* \geq m_k^*$.
\end{corollary}

Corollary \ref{cor:local-optimal} states that a device with lower marginal cost has higher utility and would contribute more data than a device with a higher marginal cost.

\begin{proof}
    With uniform payoff functions, each device $i$'s utility and utility derivative become
    \begin{equation}
        \label{eq:corollary1}
        u_i(m_i) = \phi(a(m_i)) - c_im_i, \quad u'_i(m_i) = \phi'(a(m_i))\cdot a'(m_i) - c_i.
    \end{equation}
    Due to $\phi_i(a(m))$ being concave and non-decreasing, its derivative $\phi'(a(m_i))\cdot a'(m_i)$ is non-negative and non-increasing.
    Let $m_k^o$ be the optimal amount of data contribution by device $k$.
    
    \textbf{Case 1: $c_j = c_k$}. 
    By \Eqref{eq:corollary1}, if $c_j = c_k$ then $0 = u_k'(m_k^o) = u_j'(m_k^o)$. This implies $m_k^o = m_j^o$ and subsequently $u_k(m_k^o) = u_j(m_k^o)$.
    
    \textbf{Case 2: $c_j < c_k$}. 
    By \Eqref{eq:corollary1}, if $c_j < c_k$, then $0 = u_k'(m_k^o) < u_j'(m_k^o)$.
    Since $\phi(a(m_i))$ is concave and non-decreasing, its derivative is non-increasing with its limit going to 0.
    Therefore, more data $\epsilon>0$ must be collected in order for $u_j'$ to reach zero (\textit{i.e.} $u_j'(m_k^o + \epsilon) = 0$).
    This implies that $m_j^o = m_k^o + \epsilon > m_k^o$.
    Furthermore, since $0 = u_k'(m_k^o) < u_j'(m_k^o)$, the utility for device $j$ is still increasing at $m_k^o$ and is fully maximized at $m_j^o$.
    This implies that $u_j(m_j^o) > u_k(m_k^o)$.
\end{proof}

\begin{reptheorem}{thm:pure-equ}
Consider a feasible mechanism $\mathcal{M}$ returning utility $[\mathcal{M}^U(m_i; \bm{m}_{-i})]_i$ to device $i$ 
    ($[\mathcal{M}^U(0; \bm{m}_{-i})]_i = 0$).
    Define the utility of a participating device $i$ as, 
    \begin{equation}
        u_i^r(m_i; \bm{m}_{-i}) := [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i - c_im_i.
    \end{equation}
    If $u_i^r(m_i, \bm{m}_{-i})$, is quasi-concave for $m_i \geq m^u_i := \inf \{m_i \; | \; [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i > 0 \}$ and continuous in $\bm{m}_{-i}$, then a pure Nash equilibrium with $\bm{m^{eq}}$ data contributions exists such that,
    \begin{equation}
        u_i^r(\bm{m^{eq}}) = [\mathcal{M}^U(\bm{m^{eq}})]_i - c_i \bm{m^{eq}}_i \geq u_i^r(m_i; \bm{m^{eq}}_{-i}) = [\mathcal{M}^U(m_i; \bm{m^{eq}}_{-i})]_i - c_i m_i  \text{ for } m_i \geq 0.
    \end{equation}
\end{reptheorem}

\begin{proof}
    We start the proof by examining two scenarios.
    
    \textbf{Case 1: $\max_{m_i} u_i^r(m_i; \bm{m}_{-i}) \leq 0$}.

    In the case where the marginal cost of producing updates $-c_i m_i$ is so large that the device utility $u_i$ will always be non-positive, 
    the best response $[B(\bm{m})]_i$ given a set of contributions $\bm{m}$ for device $i$ is,
    \begin{equation}
        [B(\bm{m})]_i = \argmax_{m_i \geq 0} u_i^r(m_i; \bm{m}_{-i}) = 0.
    \end{equation}
    As expected, device $i$ will not perform any updates $\bm{m^{eq}}_i = 0$.
    Therefore, \Eqref{eq:pure-eq} is fulfilled since as $\max_{m_i} u_i^r(m_i; \bm{m}_{-i}) \leq 0$ we see,
    \begin{equation}
        [\mathcal{M}^U(\bm{m^{eq}})]_i - c_i \bm{m^{eq}}_i = [\mathcal{M}^U(0; \bm{m}_{-i})]_i - c_i (0) = 0 \geq [\mathcal{M}^U(m_i; \bm{m^{eq}}_{-i})]_i - c_i m_i \text{ for all } m_i \geq 0.
    \end{equation}

    \textbf{Case 2: $\max_{m_i} u_i(m_i; \bm{m}_{-i}) > 0$}.
    
    Denote $m^u_i := \inf \{m_i \; | \; [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i > 0 \}$.
    On the interval of integers $m_i \in [0, m^u_i]$, device $i$ 's utility is non-positive, 
    \begin{equation}
        u_i^r(m_i; \bm{m}_{-i}) = [\mathcal{M}^U(m_i; \bm{m_{-i}})]_i - c_i m_i = - c_i m_i \leq 0, \quad \forall m_i \in [0, m^u_i].
    \end{equation}
    For $m_i \geq m^u_i$, we have that $u_i(m_i; \bm{m})$ is quasi-concave.
    Let the best response for a given set of contributions $\bm{m}_{-i}$ for device $i$ be formally defined as,
    \begin{equation}
        \label{eq:best-response}
        [B(\bm{m})]_i := \argmax_{m_i \geq 0} u_i^r(m_i; \bm{m}_{-i}) = \argmax_{m_i \geq 0} [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i - c_im_i.
    \end{equation}
    Suppose there exists a fixed point $\bm{\tilde{m}}$ to the best response, $\bm{\tilde{m}} \in B(\bm{\tilde{m}})$. 
    This would mean that $\bm{\tilde{m}}$ is an equilibrium since by \Eqref{eq:best-response} we have for any $m_i \geq 0$,
    \begin{equation}
        \label{eq:best-response-eq}
        [\mathcal{M}^U(\tilde{m}_i; \bm{\tilde{m}}_{-i})]_i - c_i\tilde{m}_i \geq [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i - c_im_i.
    \end{equation}
    Thus, now we must show that $B$ has a fixed point (which is subsequently an equilibrium).
    To do so, we first determine a convex and compact search space.
    As detailed in Case 1, $u_i^r(0, \bm{m}_{-i}) = 0$. 
    Therefore, we can bound $0 \leq \max_{m_i} u_i^r(m_i, \bm{m}_{-i})$.
    Since $\mathcal{M}$ is feasible, $\mathcal{M}(\bm{m})$ is bounded above by $\mathcal{M}^U_{max}$.
    Thus, we find
    \begin{equation}
        0 \leq \max_{m_i} u_i^r(m_i; \bm{m}_{-i}) \leq \mathcal{M}^U_{max} - c_i m_i.
    \end{equation}
    Rearranging yields $m_i \leq \mathcal{M}^U_{max} / c_i$.
    Since $m_i \geq m_i^u$, we can restrict our search space to $\mathcal{C} := \prod_j [m_j^u, \mathcal{M}^U_{max} / c_j] \subset \R^n$, where our best response mapping is now over $B: \mathcal{C} \rightarrow 2^\mathcal{C}$.

\begin{lemma}[Kakutani's Theorem]\label{lem:kakutani}
    Consider a multi-valued function $F : \mathcal{C} \rightarrow 2^{\mathcal{C}}$ over convex and compact domain $\mathcal{C}$ for which the output set $F(\bm{m})$ (i) is convex and closed for any fixed $\bm{m}$, and (ii) changes continuously as we change $\bm{m}$. For any such $F$, there exists a fixed point $\bm{m}$ such that $\bm{m} \in F(\bm{m})$.
\end{lemma}
    
    Since within this interval of $m_i$ $u_i^r(m_i, \bm{m}_{-i})$ is quasi-concave, $B(\bm{m})$ must be continuous in $\bm{m}$ (from \citet{acemoglu2009}).
    Now by applying Lemma \ref{lem:kakutani}, Kakutani’s fixed point theorem, there exists such a fixed point $\bm{\tilde{m}}$ such that $\bm{\tilde{m}} \in B(\bm{\tilde{m}})$ where $\bm{\tilde{m}}_i \geq m^u_i$.
    Since $\max_{m_i} u_i^r(m_i; \bm{m}_{-i}) > 0$ and $u_i^r(m_i; \bm{m}_{-i}) \leq 0$ for $m_i \in [0, m_i^u]$, $\bm{\tilde{m}}_i$ is certain to not fall within $[0, m_i^u] \; \forall i$  due to the nature of the arg max in \Eqref{eq:best-response}.
    Therefore, \Eqref{eq:best-response-eq} holds as the fixed point $\bm{\tilde{m}}$ exists and is the equilibrium of $\mathcal{M}$.
\end{proof}

\begin{reptheorem}{thm:acc-shaping}
Consider a device $i$ with marginal cost $c_i$ and accuracy payoff function $\phi_i$ satisfying Assumption \ref{assum:a2}. Denote device $i$'s optimal local data contribution as $m_i^o$ and its subsequent accuracy $\bar{a} = a(m_i^o)$. 
Define the derivative of $\phi_i(a)$ with respect to $a$ as $\phi_i'(a)$.
For any $\epsilon \rightarrow 0^+$ and marginal server reward $r(\bm{m}) \geq 0$, device $i$ has the following accuracy-shaping function $\gamma_i(m)$ for $m \geq m_i^o$,
\begin{align}
    \gamma_i := \begin{cases} \frac{-\phi_i'(\bar{a}) + \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a})(c_i - r(\bm{m}) + \epsilon) (m-m_i^o)}}{\phi_i''(\bar{a})} & \text{if } \phi_i''(\bar{a}) > 0\\
    \frac{(c_i - r(\bm{m}) + \epsilon)(m-m_i^o)}{\phi_i'(\bar{a})} & \text{if } \phi_i''(\bar{a}) = 0
    \end{cases}
\end{align}
Given the defined $\gamma_i(m)$, the following inequality is satisfied for $m \in [m_i^o, m_i^*]$,
\begin{equation}
\phi_i(a(m_i^o) + \gamma_i(m)) - \phi_i(a(m_i^o)) > (c_i - r(\bm{m}))(m - m_i^o).
\end{equation}
The new optimal contribution is $m_i^* := \{ m \geq m_i^o \; | \; a(m + \sum_{j \neq i} m_j)  =  a(m_i^o) + \gamma_i(m)\}$.
Accuracy shaping improves device $i$'s data contribution $m_i^* \geq m_i^o$ for any contribution $\bm{m}_{-i}$.
%Given all other device data contributions $\bm{m}_{-i}$, accuracy shaping improves device utility and results in a new optimal contribution $m_i^* \geq m_i^o$.
\end{reptheorem}

\begin{proof}
By the mean value version of Taylor's theorem we have,
    \begin{equation}
        \phi_i(\bar{a} + \gamma_i) = \phi_i(\bar{a}) + \gamma_i \phi_i'(\bar{a}) + 1/2 \gamma_i^2 \phi_i''(z), \quad \text{for some } z \in [\bar{a}, \bar{a} + \gamma_i].
    \end{equation}
    Since $\phi_i(a)$ is both increasing and convex with respect to $a$,
\begin{align}
    \phi_i(\bar{a} + \gamma_i) - \phi_i(\bar{a}) 
    \geq \gamma_i \phi_i'(\bar{a}) + 1/2 \gamma_i^2 \phi_i''(\bar{a}).
\end{align}
In order to ensure $\phi_i(\bar{a} + \gamma) - \phi_i(\bar{a}) > (c_i - r(\bm{m}))(m-m_i^o)$, we must select $\gamma$ such that,
\begin{equation}
\label{eq:g-ineq}
   \gamma_i \phi_i'(\bar{a}) + 1/2 \gamma_i^2 \phi_i''(\bar{a}) > (c_i - r(\bm{m}))(m-m_i^o).
\end{equation}
\textbf{Case 1: $\phi_i''(\bar{a}) = 0$.}
In this case, \Eqref{eq:g-ineq} becomes,
\begin{equation}
   \gamma_i \phi_i'(\bar{a}) > (c_i - r(\bm{m}))(m-m_i^o).
\end{equation}
In order for \Eqref{eq:g-ineq}, and thereby \Eqref{eq:gamma-satisfy}, to hold we select $\epsilon \rightarrow 0^+$ such that,
\begin{equation}
    \gamma_i := \frac{(c_i  - r(\bm{m}) + \epsilon)(m-m_i^o)}{\phi_i'(\bar{a})}.
\end{equation}

\textbf{Case 2: $\phi_i''(\bar{a}) > 0$.}
Determining when the left- and right-hand sides of \Eqref{eq:g-ineq} are equal is equivalent to solving the quadratic equation for $\gamma_i$,
\begin{align}
    \gamma_i &= \frac{-\phi_i'(\bar{a}) \pm \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a})(c_i - r(\bm{m}))(m-m_i^o)}}{\phi_i''(\bar{a})}\\
    &= \frac{-\phi_i'(\bar{a}) + \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a})(c_i - r(\bm{m}))(m-m_i^o)}}{\phi_i''(\bar{a})}.
\end{align}
The second equality follows from $\gamma_i$ having to be positive.
In order for \Eqref{eq:g-ineq}, and thereby \Eqref{eq:gamma-satisfy}, to hold we select $\epsilon \rightarrow 0^+$ such that,
\begin{equation}
    \gamma_i := \frac{-\phi_i'(\bar{a}) + \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a})(c_i -r(\bm{m}) + \epsilon) (m-m_i^o)}}{\phi_i''(\bar{a})}
\end{equation}
As a quick note, for $m = m_i^o$ one can immediately see that $\gamma_i(m) = 0$.
To finish the proof, now that \Eqref{eq:gamma-satisfy} is proven to hold for the prescribed $\gamma_i$, device $i$ is incentivized to contribute more as the added utility $\phi_i(\bar{a} + \gamma_i) - \phi_i(\bar{a})$ is larger than the incurred cost $(c_i - r(\bm{m}))(m - m_i^o)$.
There is a limit to this incentive, however.
The maximum value that $\gamma_i$ can be is bounded by the accuracy from all contributions: $a(m_i^o) + \gamma_i \leq a(\sum_j m_j)$.
Thus, device $i$ reaches a new optimal contribution $m_i^*$ which is determined by,
\begin{equation}
    \label{eq:acc-shape-interval}
    m_i^* := \{ m \geq m_i^o \; | \; a(m + \sum_{j \neq i} m_j)  =  a(m_i^o) + \gamma_i(m)\} \geq m_i^o.
\end{equation}
\end{proof}

\begin{reptheorem}{thm:main}
Our realistic federated mechanism $\mathcal{M}$, defined in \Eqref{eq:mech}, performs accuracy-shaping with $\gamma_i$ defined in Theorem \ref{thm:acc-shaping} for each device $i \in [n]$ and some small $\epsilon \rightarrow 0^+$. 
    As such, $\mathcal{M}$ is Individually Rational (IR) and has a unique Nash equilibrium at which device $i$ will contribute $m_i^* \geq m_i^o$ updates, thereby eliminating the free-rider phenomena.
    Furthermore, since $\mathcal{M}$ is IR, devices are incentivized to participate as they gain equal to or more utility than by not participating.
\end{reptheorem}

\begin{proof}
    We first prove existence of a unique Nash equilibrium by showcasing how our mechanism $\mathcal{M}$ fulfills the criteria laid out in Theorem \ref{thm:pure-equ}.
    The criteria in Theorem \ref{thm:pure-equ} largely surrounds the utility of a participating device $i$,
    \begin{equation}
        \label{eq:util-quasiconcave}
        u_i^r(m_i; \bm{m}_{-i}) := [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i - c_im_i.
    \end{equation}

    \textbf{Feasibility.} Before beginning, we note that $\mathcal{M}$ trivially satisfies the only non-utility requirement that $[\mathcal{M}^U(0; \bm{m}_{-i})]_i = 0$ (as $a(0) = \phi_i(0) = 0$).
    As shown in \Eqref{eq:mech}, $\mathcal{M}$ returns accuracies between 0 and $a(\sum \bm{m})$ to all devices.
    This satisfies the bounded accuracy requirement.
    Furthermore, the utility provided by our mechanism $\mathcal{M}^U$ is bounded as well.
    Since $a_{opt}$ is the largest attained accuracy by our defined accuracy function $\hat{a}(m)$ and $a_{opt}<1$, the maximum utility is $\phi_i(a_{opt}) < \infty$.
    Now, that $\mathcal{M}$ is proven to be Feasible, we only need the following to prove that $\mathcal{M}$ has a pure equilibrium: \textbf{(1)} $u_i^r(m_i; \bm{m}_{-i})$ is continuous in $\bm{m}_{-i}$ and \textbf{(2)} quasi-concave for $m_i \geq m^u_i := \inf \{m_i \; | \; [\mathcal{M}^U(m_i; \bm{m}_{-i})]_i > 0 \}$.

    \textbf{Continuity.} By definition of $u_i^r(m_i; \bm{m}_{-i})$, \Eqref{eq:util-quasiconcave}, we only need to consider 
    $[\mathcal{M}^U(m_i; \bm{m}_{-i})]_i$ since that is the only portion affected by $\bm{m}_{-i}$.
    By definition of the utility returned by our mechanism $\mathcal{M}$, shown in \Eqref{eq:mech-utility}, no discontinuities arise for a fixed $m_i$ and varying $\bm{m}_{-i}$.
    By assumptions on continuity in Assumptions \ref{assum:a1} and \ref{assum:a2}, $\phi_i(a(m))$ is continuous for all $m$.
    Thus, for non-zero utility (zero utility would lead to zero reward), we find the marginal monetary reward function $r(\bm{m})$ in \Eqref{eq:server-reward} is continuous.
    Therefore, each piecewise component of $[\mathcal{M}^U(m_i; \bm{m}_{-i})]_i$ is continuous since they are sums of continuous functions.
    Finally, we show that the piecewise functions connect with each other continuously.
    The accuracy-shaping function $\gamma_i$ is defined such that $\gamma_i(m_i^o) = 0$ and $a(m_i^o) + \gamma_i(m_i^*) = a(\sum \bm{m})$, which finishes proof of continuity.
    
    
    %$\mathcal{M}$ remains continuous regardless of the contribution $\bm{m}_{-i}$ from all devices outside of device $i$. 
    %As $\bm{m}_{-i}$ changes, the values of $r(\bm{m})$ and $m_i^*$ change.
    %The changes to $m_i^*$ only affect the interval of accuracy shaping (larger $\bm{m}_{-i}$ invokes a larger $m_i^*$ by \Eqref{eq:acc-shape-interval}).
    %Changes to $r(\bm{m})$ can affect the outputted utility $[\mathcal{M}^U(\bm{m})]_{i}$, however the outputted utilities remain continuous due to the max operator (which ensures continuity since the functions within the max operator are continuous).

    \textbf{Quasi-Concavity.}
    For all values of $m_i \geq m^u_i$, our mechanism $\mathcal{M}$ produces positive utility.
    By construction, our mechanism $\mathcal{M}$ is strictly increasing for $m_i \geq m^u_i$.
    Our mechanism $\mathcal{M}$ returns varying utilities within three separate intervals.
    While piece-wise, these intervals are continuous and $\mathcal{M}$ is strictly increasing with respect to $m_i$ in each.
    The first interval, consisting of the concave function $\phi_i(a(m_i))$, is quasi-concave by construction.
    The second interval consists of a linear function $r(\bm{m}) \cdot (m_i-m_i^o)$ added to a quasi-concave  $\phi_i(a(m_i) + \gamma_i(m_i))$ function, resulting in a quasi-concave function (note that $\phi_i(\hat{a}(m_i))$ is concave).
    Finally, the third interval consists of a linear function $r(\bm{m}) \cdot (m_i-m_i^*)$ added to a concave function $\phi_i(a(m_i))$, which is also quasi-concave.
    In sum, this makes $[\mathcal{M}^U(m_i; \bm{m}_{-i})]_i$ a quasi-concave function.
    Since $-c_i m_i$ is a linear function, the utility of a participating device $u_i^r(m_i; \bm{m}_{-i})$ will also be quasi-concave function, as the sum of a linear and quasi-concave function is quasi-concave.

    \textbf{Existence of Pure Equilibrium with Increased Data Contribution.}
    Since $[\mathcal{M}^U(\bm{m})]_{i}$ satisfies feasibility, continuity, and quasi-concavity requirements, $\mathcal{M}$ is guaranteed to have a pure Nash equilibrium by Theorem \ref{thm:pure-equ}.
    Furthermore, since $\mathcal{M}$ performs accuracy-shaping with $\gamma_i$ prescribed in Theorem \ref{thm:pure-equ}, it is guaranteed that each device $i$ will produce $m_i^* \geq m_i^o$ updates.

    \textbf{Individually Rational (IR).} We prove $\mathcal{M}$ is IR by looking at each piecewise portion of \Eqref{eq:mech}:

    \textit{Case 1: $m_i \leq m_i^o$ (Free-Riding).}
    When $m_i \leq m_i^o$, a device would attempt to provide as much or less than the amount of contribution which is locally optimal.
    The hope for such strategy would be free-riding: enjoy the performance of a well-trained model as a result of federated training while providing few (or zero) data points in order to save costs.
    Our mechanism avoids the free rider problem trivially by returning a model with an accuracy that is proportional to the amount of data contributed by the device.
    This is shown in \Eqref{eq:mech}, as devices receive a model with accuracy $a(m_i)$ if $m_i \leq m_i^o$ (\textit{i.e.,} devices are rewarded with a model equivalent to one that they could've trained themselves if they fail to contribute an adequate amount of data).
    In this case, devices receive the same model accuracy as they would've on their own and thus IR is satisfied in this case.

    \textit{Case 2: $m_i \in (m_i^o , m_i^*]$.}
    Via the results of Theorem \ref{thm:acc-shaping}, the accuracy of the model returned by $\mathcal{M}$ when $m_i \in (m_i^o , m_i^*]$ is greater than a model trained by device $i$ on $m_i$ local contributions.
    Mathematically this is described as $a^r(m_i) = a(m_i) + \gamma_i(m_i) > a(m_i)$ for $m_i \in (m_i^o , m_i^*]$.
    Since $\phi_i$ is increasing, this ensures that \Eqref{eq:ir} holds.
    %Through the use of the max operator, it is guaranteed that \Eqref{eq:mech} will also satisfy \Eqref{eq:ir}.

    \textit{Case 3: $m_i \geq m_i^*$.}
    By Theorem \ref{thm:acc-shaping}, by definition of $m_i^*$ when $m_i = m_i^*$ then the accuracy of a returned model by $\mathcal{M}$ is equal to $a(\sum_j m_j)$.
    Therefore, given a fixed set of contributions from all other devices $\bm{m_{-i}}$, device $i$ will still attain a model with accuracy $a(\sum_j m_j)$ for $m_i \geq m_i^*$ (since the limits of accuracy shaping have been reached for the given contributions).
    Due to this, \Eqref{eq:ir} trivially holds as $a(\sum_j m_j) \geq a(m_i)$.
\end{proof}


\subsection{Accuracy Modeling}
\label{app:acc-modeling}

Our model for accuracy stems from Example 2.1 in \citet{karimireddy2022mechanisms}, which in turn comes from Theorem 11.8 in \citet{mehryar2019}.
Below is the mentioned generalization bound,
\begin{proposition}[Generalization Bounds, 
\citet{karimireddy2022mechanisms} Example 2.1]
    Suppose we want to learn a model $h$ from a hypothesis class $\gH$ which minimizes the error over data distribution $\gD$, defined to be $R(h) := \mathbb{E}_{(x,y) \sim \gD}[e(h(x), y)]$, for some error function $e(\cdot) \in [0, 1]$. Let such an optimal model have error $(1 - a_{opt}) \leq 1$. Now, given access to $\{(x_l, y_l)\}l \in [m]$ which are m i.i.d. samples from $\gD$, we can compute the empirical risk minimizer (ERM) as $\hat{h}_m = \argmin_{h \in \gH} \sum_{l \in [m]} e(h(x), y)$. Finally, let $k>0$ be the pseudo-dimension of the set of functions $\{(x, y) \rightarrow e(h(x), y) : h \in \gH \}$, which is a measure of the difficulty of the learning task. Then, standard generalization bounds imply that with probability at least 99\% over the sampling of the data, the accuracy is at least
    \begin{equation}
    \label{eq:gen-bound2}
        1 - R(\hat{h}_m) \geq \bigg\{\hat{a}(m) := a_{opt} - \frac{\sqrt{2k(2 + \log (m/k))}+4}{\sqrt{m}} \bigg \}.
    \end{equation}
    A simplified expression for our analytic analysis use is,
    \begin{equation}
    \label{eq:acc2}
        \hat{a}(m) = a_{opt} - 2\sqrt{k/m}.
    \end{equation}
\end{proposition} 



==> old/a2-experiments.tex <==
\section{Experimental Results Continued}
\label{app:exp}

In this section we provide durther details into how our image classification experiments were run.
As a note, we ran each experiment three times, varying the random seeds.
All bar plots in our paper showcase the mean results of the three experiments.
In Figures \ref{fig:acc-plots-16} and \ref{fig:acc-plots-8}, we plot error bars.
The error bars are quite thin, as the results did not vary much between each of the three experiments.

\subsection{Additional Experimental Details}

\textbf{Experimental Setup.}
Within our experiments, both $8$ and $16$ devices train a ResNet18 and a small convolutional neural network for CIFAR-10 and MNIST respectively.
As detailed in Appendix \ref{app:exp}, we carefully select and tune $a_C(m)$ to match the empirical training results on both datasets as closely as possible.
Once tuned, we select a fixed marginal cost $c_e$ of 2.5e-4 (4e-5) for CIFAR-10 (MNIST) on all baselines.
When performing uniform cost experiments, each device uses $c_e$ as its marginal cost (and thus each device has the same amount of data).
For non-uniform cost experiments, $c_e$ is the mean of a Gaussian distribution from which the marginal costs are sampled.
Our uniform accuracy payoff is $\phi_i(a) = \frac{1}{(1-a)^2} - 1$ for each device $i$.
For non-uniform payoff experiments, we set $\phi_i(a) = z_i(\frac{1}{(1-a)^2} - 1)$ where $z_i$ is uniformly sampled within $[0.9, 1.1]$.
Additional experiments and details are found in Appendix \ref{app:exp}.

\textbf{Experimental Process.}
The experimental process involved careful tuning of our theoretical accuracy function $\hat{a}(m)$ in order to match the empirical accuracy results we found.
In fact, for CIFAR-10 we use $\hat{a}(m)$ defined in \Eqref{eq:gen-bound} with carefully selected values for $k$ and $a_{opt}$ to precisely reflect the empirical results found for our CIFAR-10 training.
For MNIST, however, an accuracy function of $\hat{a}(m) = a_{opt} - 2 \sqrt{k/m}$ was more reflective of the ease of training on MNIST.
Overall, to ensure precise empirical results, we followed the following process for each experiment (for both CIFAR-10 and MNIST as well as for 8 and 16 devices):
\begin{enumerate}[leftmargin=*]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \item Determine $a_{opt}$ and $k$ such that $\hat{a}(m)$ is tuned to most precisely reflect our empirical results.
    \item Select an amount of data that each device should have \textit{in expectation of varying costs and payoffs} (this amount should ensure that there is enough unique datapoints to share amongst devices).
    \item From the prescribed amount of data and $a(m)$, derive the marginal cost $c_e$ required to produce the desired data quantity.
    \item For non-uniform experiments, draw a marginal cost at random from a Gaussian with mean $c_e$ and/or draw a payoff function $\phi_i$ with a $z_i$ sampled within $[0.9, 1.1]$ (detailed in Section \ref{sec:experiments}).
    \item Save an initial model for training.
    \item Train this initial model locally on each device until convergence, generating $a_{local}$.
    \item Using the initial model, train the model in a federated manner until convergence, generating $a_{fed}$.
    \item Using the accuracy-shaping function, compute the amount of additional data contributions required to raise $a_{local}$ to $a_{fed}$. \textit{This is the incentivized amount of added contributions}.
\end{enumerate}
% We select $\tau$ such that all devices, which we assume to be homogeneous (a realistic assumption since they are all processes from the same cluster), complete 6 FedAvg steps before returning the model for averaging to the server.
We also use the expected payoff function for the central server: $\phi_C = 1/(1-a)^2 - 1$.
Within experiments, for simplicity, we set the profit margin $p_m = 1$ (greedy server).
Below, we detail the hyper-parameters used in our CIFAR-10 and MNIST experiments.

\begin{table}[H]
\caption{Hyper-parameters for CIFAR-10 Experiments.}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Model    & Batch Size & Learning Rate & $a_{opt}$ & $k$ & Epochs & Local FedAvg Steps $h$ \\ \hline
ResNet18 & 128        & 1e-3          & 0.9       & 18  & 100    & 6           \\ \hline
\end{tabular}
\end{table}


\begin{table}[H]
\caption{Hyper-parameters for MNIST Experiments.}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Model    & Batch Size & Learning Rate & $a_{opt}$ & $k$ & Epochs & Local FedAvg Steps $h$ \\ \hline
CNN & 128        & 1e-3          & 0.995       & 0.25  & 50    & 6           \\ \hline
\end{tabular}
\end{table}

\subsection{Additional Experimental Results}

It is interesting to note how well \realfm performs on MNIST (in terms of the vastly improved utility seen in Figures \ref{fig:mnist-server-16} and \ref{fig:mnist-server-8}) while FedAvg only improves model accuracy by a mere couple of percentage points.
The reason stems from the payoff function $\phi_i$ which heavily rewards models that have accuracies close to 100\%.
This scenario is rational in real-world settings.
Competing companies in industry will all likely have models which are high-performing (above 95\% accuracy).
Since the competition is stiff, companies with the best model performance will likely attract the most customers since their product is the best.
Therefore, the utility for achieving model performance close to 100\% should become larger and larger as one gets closer to 100\%.

\input{figures/accuracy-plots-16}

\textbf{8 Device Image Classification Results.}
Below we provide CIFAR-10 and MNIST results for 8 devices.
These plots mirror those shown in Section \ref{sec:experiments} for 16 devices.
In both cases, we find that utility sharply improves for the central server and participating devices.
Data contribution also improves for CIFAR-10 and MNIST.
Under all scenarios \realfm performs the best compared to all other baselines.
First, we start with the test accuracy curves for both datasets.

\input{figures/accuracy-plots-8}

\input{figures/cifar-server-8}

\input{figures/mnist-server-8}

\input{figures/device-utility-8}


==> sections/0-Abstract.tex <==
\begin{abstract}
Edge device participation in federating learning~(FL) is typically studied through the lens of device-server communication (\textit{e.g.,} device dropout) and assumes an undying desire from edge devices to participate in FL.
As a result, current FL frameworks are flawed when implemented in realistic settings, with many encountering the free-rider dilemma.
In a step to push FL towards realistic settings, we propose \realfm: the first federated mechanism that (1) realistically models device utility, (2) incentivizes data contribution and device participation, (3) provably removes the free-rider dilemma, and (4) relaxes assumptions on data homogeneity and data sharing.
Compared to previous FL mechanisms, \realfm allows for a non-linear relationship between model accuracy and utility, which improves the utility gained by the server and participating devices.
On real-world data, \realfm improves device and server utility, as well as data contribution, \textit{by over $3$ and $4$ magnitudes} respectively compared to baselines.
% Code for \realfm is found on GitHub at \url{https://github.com/umd-huang-lab/RealFM}.
\end{abstract}

==> sections/1-Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Federated Learning (FL) is a collaborative framework where, in the \emph{cross-device} setting, edge devices jointly train a global model by sharing locally computed model updates with a central server.
It is generally assumed within FL literature that edge devices will (i) always participate in training and (ii) use all of its local data during training. 
However, it is irrational for devices to participate in, and incur the costs of, federated training without receiving proper benefits back from the server (via model performance or monetary rewards).
Specifically, there are two major challenges:

\textbf{(C1) Lack of Participation Incentives}.
Current FL frameworks generally lack incentives to increase device participation.
This leads to training with fewer devices and data to compute local updates, which can potentially reduce model accuracy.
Incentivizing devices to participate in training and produce more data, especially from a server's perspective, improves model performance (further detailed in Section \ref{sec:formulation}), which leads to greater utility for both the devices and server.

\textbf{(C2) Lack of Contribution Incentives: The Free-Rider Dilemma}.
In realistic settings, devices determine their own optimal amount of data usage for federated contributions.
As such, many FL frameworks run the risk of encountering the free-rider problem: devices do not contribute gradient updates yet reap the benefits of a well-trained collaborative model. 
Removing the free-rider effect in FL frameworks is critical because it improves performance of trained models \citep{wang2023frad, wang2022assessing} and reduces security risks \citep{fraboni2021free, lin2019free, wang2022pass} for devices. 

To address these challenges, a handful of recent FL literature \citep{karimireddy2022mechanisms, zhan2020learning, zhan2020big, zhan2021incentive} consider device \textbf{utility}: the net benefit received by a device for participating in federated training.
Every rational device $i$ aims to maximize its utility $u_i$.
Consequently, utility is the guiding factor in whether rational devices participate in federated training.
Devices will only participate if the utility $u_i^r$ gained, via its rewards $(a^r_i, R_i)$, outstrips the maximum utility gained from local training $u_i^o$.
In a step towards more realistic FL, the referenced works \citep{karimireddy2022mechanisms, zhan2020learning, zhan2020big, zhan2021incentive} design mechanisms, or systems, that maximize device utility, and provide greater utility than local training, when more data is contributed.

% devices contribute more data and participate in training.
% derive participation and optimal data usage via \textit{maximization} of device utility.


While previous FL works incorporate utility, they require \textbf{unrealistic assumptions} such as disallowing \textbf{(i)} devices having utility that depends non-linearly on their model accuracy, \textbf{(ii)} heterogeneous data distributions across devices, \textbf{(iii)} truly federated (non-data sharing) methods, and \textbf{(iv)} modeling of central server utility.
%\fhst{a non-linear relationship between model accuracy and utility,} 
In our paper, we take a leap towards realistic federated systems by relaxing all 4 assumptions above while simultaneously solving the %\fhst{following} 
key issues in \textbf{C1} and \textbf{C2}.



\input{figures/mechanism-diagram}


\textbf{Summary of Contributions}.
We propose \realfm: a federated mechanism $\mathcal{M}$ (\textit{i.e.,} system) that a server, in a FL setup, implements to eliminate \textbf{(C1)} and \textbf{(C2)} when rational devices participate. 
\realfm is \textit{Individually Rational} (IR): participating devices and the server provably receive greater utility than training alone $u_i^r \geq u_i^o$.
The goal of \realfm is to \textit{design a reward protocol, with model-accuracy $a^r$ and monetary $R$ rewards, such that rational devices choose to participate and contribute more data.}
By increasing device participation and data contribution, a server trains a higher-performing model and subsequently attains greater utility.
\realfm is a mechanism that,
\vspace{-4mm}
\begin{itemize}[itemsep=0in,leftmargin=*]
    \item eliminates \textbf{(C1)} and \textbf{(C2)}, i.e., provably eliminates the free-rider effect by incentivizing devices to participate and use more data during the federated training process than they would on their own,
    \item allows more \textbf{realistic settings}, including: \textbf{(1)} a non-linear relationship between accuracy and utility, \textbf{(2)} data heterogeneity, \textbf{(3)} no data sharing, and  \textbf{(4)} modeling of central server utility.
%(via a properly modeling of device utility)
 \item produces state-of-the-art results towards improving utility (for both the server and devices), data contribution, and final model accuracy on real-world datasets.
%\vspace{-4mm}
\end{itemize}

    
% \vspace{-4mm}
%\begin{enumerate}[itemsep=0in,leftmargin=0.5in]
%\setlength{\itemsep}{1pt}
%\setlength{\parskip}{0pt}
%\setlength{\parsep}{0pt}
%\item a non-linear relationship between accuracy and utility (via a properly modeling of device utility), 
% thereby improving both server and device utility,
% relaxing assumptions to allow for
%\item modeling of central server utility, 
    %\item data heterogeneity, 
%\item not required data sharing, 
%\end{enumerate}

%\fhc{Sorry I messed with the format here.}
 
%We propose \realfm: a federated mechanism $\mathcal{M}$ (\textit{i.e.,} game) that a server, in a FL setup, implements to eliminate \textbf{(C1)} and \textbf{(C2)} when rational devices participate. 
%\textit{The goal of \realfm is to design a reward protocol, with model-accuracy $a^r$ and monetary $R$ rewards, such that rational devices choose to participate and contribute more data.}
%By increasing device participation and data contribution, a server trains a higher-performing model and subsequently attains greater utility.
%
%\textbf{Summary of Contributions}. 
%We propose an \textit{Individually Rational} (IR) federated mechanism \realfm, which means (i) the server provably achieves increased utility and (ii) devices are guaranteed to receive rewards, through mechanism participation, that provide greater utility than local training $u_i^r \geq u_i^o$.
%\realfm improves upon previous federated mechanisms by:


% Only a small handful of recent FL literature \citep{karimireddy2022mechanisms, zhan2020learning, zhan2020big, zhan2021incentive} consider device \textbf{utility}: the net benefit received by a device for participating in federated training.
% In a step towards more realistic federated systems, these works derive participation and optimal data usage via \textit{maximization} of device utility.

%Utility is the backbone of realistic FL settings. 

%In realistic settings, device utility is personal: each device relates model accuracy $a$ to utility with a unique function $\phi_i$ and has a personal training cost $c_i$.

==> sections/2-Related-Works.tex <==
\section{Related Works}
\label{sec:related-works}

\textbf{Federated Mechanisms.}
Previous literature \citep{chen2020mechanism, zhan2020learning, zhan2020big, zhan2021incentive} have proposed mechanisms to solve \textbf{(C1)} and incentivize devices to participate in FL training.
However, these works fail to address \textbf{(C2)}, the free-rider problem, and have unrealistic device utilities.
In \citet{chen2020mechanism}, data sharing is allowed, which is prohibited in the FL setting due to privacy concerns.
% , as one of the main motivations of FL is to train models in a privacy-preserving manner
In \citet{zhan2020learning, zhan2020big, zhan2021incentive}, device utility incorporates a predetermined reward for participation in federated training without specification on how this amount is set by the server.
This could be unrealistic, since rewards should be dynamic and depend upon the success (resulting model accuracy) of the federated training.
Setting too low of a reward impedes device participation, while too high of a reward reduces the utility gained by the central server (and risks negative utility if performance lags total reward paid out).
Overall, predicting an optimal reward \textit{prior} to training is unrealistic.
In contrast, our proposed \realfm introduces a principled mechanism to set the rewards.

The recent work by \citet{karimireddy2022mechanisms} is the first to simultaneously solve \textbf{(C1)} and \textbf{(C2)}.
They propose a mechanism that incentivize devices to (i) participate in training and (ii) produce more data than on their own (data maximization).
By incentivizing devices to maximize production of local data, the free-rider effect is eliminated.
While this proposed mechanism is a great step forward for realistic mechanisms, pressing issues remain. 
First, \citet{karimireddy2022mechanisms} requires data sharing between devices and the central server.
This is acceptable if portions of local data are shareable (\textit{i.e.} no privacy risks exist for certain subsets of local data), yet it violates the key tenet of FL: privacy.
% yet it runs counter to the original draw of FL: a privacy-preserving training method which \textit{does not require} devices share data with the server.
Second, device utility is designed in \citet{karimireddy2022mechanisms} such that the utility improves linearly with increasing accuracy.
%We find this unrealistic, as an increase in model accuracy from $49$\% to $50$\% should not hold the same utility as an increase from $98$\% to $99$\%.
We find this unrealistic, as devices likely find greater utility for an increase in accuracy from $98$\% to $99$\% than $48$\% to $49$\%.
Finally, \citet{karimireddy2022mechanisms} assumes all local data comes from the same distribution, which is unrealistic.
Our proposed \realfm addresses all issues above.
Further discussion is in Appendix \ref{app:notation}.

\textbf{Contract Theory and Federated Free Riding.}
Contract theory in FL aims to optimally determine the balance between device rewards and registration fees (cost of participation).
In contract mechanisms, devices may sign a contract from the server specifying a task, reward, and registration fee.
If agreed upon, the device signs and pays the registration fee.
Each device receives the reward if it completes the task and receives nothing if it fails.
Contract mechanisms have the ability to punish free riding in FL by creating negative incentive if a device does not perform a prescribed task (\textit{i.e.,} it will lose its registration fee).
The works \cite{cong2020game, kang2019incentive, lim2020hierarchical, lim2021towards, liu2022contract, wang2021federated} propose such contract-based FL frameworks.
While effective at improving model generalization accuracy and utility \citep{lim2020hierarchical, liu2022contract}, 
these works focus on optimal reward design.
Our \realfm mechanism does not require registration fees, boosting device participation, and utilizes an accuracy shaping method to provide rewards at the end of training in an optimal and more realistic approach. 
Furthermore, like \citet{karimireddy2022mechanisms}, our mechanism incentivizes increased contributions to federated training, which is novel compared with the existing contract theory literature and mechanisms.
\vspace{-3mm}

==> sections/5-Realistic-Mechanism-arxiv.tex <==
\section{\realfm: A Step Towards Realistic Federated Mechanisms}
\label{sec:fed-mech}
We reiterate that the goal of our proposed \realfm mechanism $\mathcal{M}_{R}$ (Algorithm \ref{alg:realfm}) is to design a reward protocol, with model-accuracy $a^r$ and monetary $R$ rewards, such that rational devices choose to participate and contribute more data than is locally optimal (Theorem \ref{thm:local-optimal}) in exchange for improved device utility.
Denote the \textit{utility} that \realfm provides to each device $i$ as $\mathcal{M}^U_{R,i} := [\mathcal{M}^U_R(\bm{m})]_i$.
\begin{align}
    \label{eq:mech}
    \mathcal{M}_R(m_i; \bm{m}_{-i}) &:= \begin{cases} \big( a_i(m_i), \; 0 \big) \quad \text{ if } m_i \!\leq \!m_i^o,\\ \big( a_i\big(m_i^o\big) + \gamma_i(m_i), \; r(\bm{m})(m_i - m_i^o) \big) \quad\text{ if } m_i \!\in\! [m_i^o, m_i^{*}],\\
    \big( a_C(\sum \bm{m}), \; r(\bm{m})(m_i - m_i^o) \big) \quad\text{ if } m_i \!\geq\! m_i^{*}.
    \end{cases}\\
    \label{eq:mech-utility}
    \mathcal{M}^U_{R, i} &:= \begin{cases}
         \phi_i \big( a_i(m_i) \big) \quad\text{ if } m_i \!\leq \!m_i^o,\\
         \phi_i \big( a_i(m_i^o) + \gamma_i(m_i) \big) + r(\bm{m})(m_i - m_i^o) \quad\text{ if } m_i \!\in\! [m_i^o, m_i^{*}], \\
          \phi_i \big( a_C(\sum \bm{m}) \big) + r(\bm{m})(m_i - m_i^{o}) \quad\text{ if } m_i \!\geq\! m_i^{*}.
    \end{cases}
\end{align}

As described mathematically above, \realfm eliminates free-riding by returning a model with accuracy equivalent to local training $a_i(m_i)$ for a device $i$ which does not contribute more than what is locally optimal ($m_i \leq m_i^o$).
This can be accomplished in practice by carefully degrading the final model with noisy perturbations (or continued training on a skewed subset of data).
Importantly, this process ensures Individually Rationality~(IR), as devices receive at least as good performance as if they had trained by themselves (\textbf{incentivizing participation}).
Devices which contribute more than

\begin{wrapfigure}{R}{0.54\textwidth}
    \vspace{-3mm}
    \begin{minipage}{0.54\textwidth}
      \input{sections/realfm-algo}
      \vspace{-10mm}
    \end{minipage}
\end{wrapfigure}

what is locally optimal receive boosted accuracy $\gamma_i(m_i)$ and monetary rewards $r(\bm{m})(m_i - m_i^o)$ up to a new federated equilibrium $m_i^*$ (detailed in Theorem \ref{thm:acc-shaping}).
This process ensures that devices are incentivized to contribute more than what is locally optimal (\textbf{incentivizing contributions}).
Finally, if devices contribute more than the new equilibrium, the server can only provide the model accuracy equivalent to the fully trained global model $a_C(\sum\bm{m})$ as well as monetary rewards  $r(\bm{m})(m_i - m_i^o)$ (\textbf{feasibility}).
Below, we detail how the accuracy $\gamma_i$ and monetary $r(\bm{m})$ rewards are constructed to ensure devices receive greater utility even when they contribute more than what is locally optimal.

\textbf{Accuracy Rewards: Accuracy Shaping}.
Accuracy shaping is responsible for incentivizing devices to collect more data than what is locally optimal $m_i^o$.
The idea behind accuracy shaping is to incentivize device $i$ to use more data $m_i^* \geq m_i^o$ for federated training by providing a boosted model accuracy whose utility outstrips the marginal cost of collecting more data $c_i \cdot \left(m_i^* - m_i^o\right)$.
Unlike \cite{karimireddy2022mechanisms}, \realfm performs accuracy with non-linear accuracy payoffs $\phi$ ($\phi$ is assumed to be linear in \cite{karimireddy2022mechanisms}).
To overcome the issues with non-linear $\phi$'s, we carefully construct an accuracy-shaping function $\gamma_i(m)$ for each device $i$.
Devices which participate in $\mathcal{M}_R$ must share $c_i, \phi_i$ with the server.

\begin{assumption}
    \label{assum:a3}
    For a given set of device contributions $\bm{m}$, the maximum accuracy attained by the server must be greater than that of any single device, $a_C(\sum \bm{m}) \geq a_{i}(m^o_{i}) \; \forall i \in [n]$.
\end{assumption}
% \vspace{-4mm}

Assumption \ref{assum:a3} states that the globally-trained model outperforms any locally-trained model from the participating devices.
This is valid if the direction of descent taken by the server is beneficial for all participating devices (\textit{i.e.,} the inner product between local gradients and the aggregated gradient is positive).
This assumption may be violated in certain non-iid settings, where a participating device's local data distribution greatly differs from the majority of devices.
We note that our experiments use various non-iid data distributions, none of which violate Assumption \ref{assum:a3}.

\begin{theorem}[Accuracy Shaping Guarantees]
\label{thm:acc-shaping}
Consider a device $i$ with marginal cost $c_i$ and accuracy payoff function $\phi_i$ satisfying Assumptions \ref{assum:a2} and \ref{assum:a3}. Denote device $i$'s optimal local data contribution as $m_i^o$ and its subsequent accuracy $\bar{a}_i := a_i(m_i^o)$. 
Define the derivative of $\phi_i(a)$ with respect to $a$ as $\phi_i'(a)$.
For any $\epsilon \rightarrow 0^+$ and marginal server reward $r(\bm{m}) \geq 0$, device $i$ has the following accuracy-shaping function $\gamma_i(m)$ for $m \geq m_i^o$,
\begin{align}
\label{eq:gamma}
    \gamma_i := \begin{cases} \frac{-\phi_i'(\bar{a}_i) + \sqrt{\phi_i'(\bar{a})^2 + 2\phi_i''(\bar{a}_i)(c_i - r(\bm{m}) + \epsilon) (m-m_i^o)}}{\phi_i''(\bar{a}_i)},\\
    %& \text{if } \phi_i''(\bar{a}_i) > 0
    \frac{(c_i - r(\bm{m}) + \epsilon)(m-m_i^o)}{\phi_i'(\bar{a}_i)} \quad \text{if } \phi_i''(\bar{a}_i) = 0
    \vspace{-3mm}
    \end{cases}
\end{align}
Given the defined $\gamma_i(m)$, the following inequality is satisfied for $m \in [m_i^o, m_i^*]$,
\begin{equation}
\label{eq:gamma-satisfy}
\phi_i(\bar{a}_i + \gamma_i(m)) - \phi_i(\bar{a}_i) > (c_i - r(\bm{m}))(m - m_i^o).
\end{equation}
%Now,  $m_i^* := \{ m \geq m_i^o \; | \; \max \{ \bar{a}_i,  a_C(m + \sum_{j \neq i} m_j) \}  =  \bar{a}_i + \gamma_i(m)\}$ is the optimal contribution for each device $i$.
Now,  $m_i^* := \{ m \geq m_i^o \; | \; a_C(m + \sum_{j \neq i} m_j)  =  \bar{a}_i + \gamma_i(m)\}$ is the optimal contribution for each device $i$.
Device $i$'s data contribution increases $m_i^* \geq m_i^o$ for any contribution $\bm{m}_{-i}$.
\end{theorem}
\vspace{-3mm}
Theorem \ref{thm:acc-shaping} (proof in Appendix \ref{app:proofs}) 
defines an accuracy-shaping function $\gamma_i$ (\Eqref{eq:gamma}) that ensures devices receive more gain in utility than loss by contributing more than is locally optimal (\Eqref{eq:gamma-satisfy}) up to a feasible equilibrium $m_i^*$ (the server cannot provide an accuracy beyond $a_C(\sum \bm{m})$).
\begin{remark}
    \label{remark5:acc-shaping}
    For a linear accuracy payoff, $\phi_i(a) = wa$ for $w>0$, \Eqref{eq:gamma} relays $\gamma_i = \frac{(c_i - r(\bm{m}) + \epsilon)(m - m_i^o)}{w}$. 
    We recover the accuracy-shaping function, Equation (13), in \citet{karimireddy2022mechanisms} with their no-reward $r(\bm{m})=0$ and $w=1$ linear setting.
    Thus, our accuracy-shaping function generalizes the one in \citet{karimireddy2022mechanisms}.
\end{remark}
\begin{remark}[Proportional Shaping]
    \label{remark6:acc-shaping}
    When local accuracy $\bar{a}_i$ is low, the values of $\phi_i'(\bar{a}_i), \phi_i''(\bar{a})$ are smaller (Assumption \ref{assum:a2}) and thus $\gamma_i(m)$ grows faster w.r.t $m$ (\Eqref{eq:gamma}).
    Thus, for a low-accuracy device $i$, $\gamma_i$ will reach its upper accuracy limit at a smaller optimal contribution $m_i^*$.
    The result is proportional shaping: contributions are incentivized in proportion to device performance.
\end{remark}
\vspace{-3mm}
\textbf{Monetary Rewards}.
As detailed in Section \ref{sec:utility}, the server keeps a fraction $p_m$ of its utility gained at the end of training (\Eqref{eq:server-utility}).
\realfm disperses the remaining $1 - p_m$ utility as a marginal monetary reward $r(\bm{m})$ for each data point contributed more than locally optimal,
\begin{equation}
    \label{eq:server-reward}
    r(\bm{m}) := (1-p_m) \cdot \phi_C\left(a_C\left(\sum \bm{m}\right)\right) / \sum \bm{m} \; \longrightarrow \; R_i := r(\bm{m})(m_i - m_i^o).
\end{equation}
The marginal monetary reward $r(\bm{m})$ is dynamic and depends upon the total amount of data used by devices during federated training.
Therefore, $r(\bm{m})$ is unknown to devices when $\mathcal{M}_R$ is issued.
However, the server computes and provides the monetary rewards once training is complete.

\begin{theorem}[Existence of Improved Equilibrium]
\label{thm:main}
    \realfm $\mathcal{M}_R$ (\Eqref{eq:mech}) performs accuracy-shaping with $\gamma_i$ defined in Theorem \ref{thm:acc-shaping} for each device $i \in [n]$ and some $\epsilon \rightarrow 0^+$. 
    As such, $\mathcal{M}_R$ is Individually Rational (IR) and has a unique Nash equilibrium at which device $i$ will contribute $m_i^* \geq m_i^o$ updates, thereby eliminating the free-rider phenomena.
    Furthermore, since $\mathcal{M}_R$ is IR, devices are incentivized to participate as they gain equal to or more utility than by not participating.
\end{theorem}
\vspace{-3mm}
Since \realfm (\textbf{i}) returns model accuracy equivalent to local training if devices do not contribute more than what is locally optimal, and (\textbf{ii}) ensures that devices are provided improved utility when contributing more than locally optimal (Theorem \ref{thm:acc-shaping}), \realfm is IR.
Furthermore, since $\mathcal{M}_R$ is feasible and the utility provided is continuous and quasi-concave (\Eqref{eq:mech-utility}), there exists a Nash equilibrium (Theorem \ref{thm:pure-equ}).
The use of accuracy shaping (Theorem \ref{thm:acc-shaping}) also ensures that devices contribute more data than is locally optimal, eliminating the free-rider effect.
Our experiments provide empirical backing that \realfm indeed  incentives devices to contribute more data and improves both device and server utility.


==> sections/6-Experiments.tex <==
\input{figures/server-utility-comparison-16}
\section{Experimental Results}
\label{sec:experiments}
To test the efficacy of \realfm, we analyze how well it performs at \textbf{(i)} improving utility for the central server and devices, and \textbf{(ii)} increasing the amount of data contributions to federated training on image classification experiments.
We perform experiments on CIFAR-10 \citep{krizhevsky2009learning} and MNIST \citep{deng2012mnist}.

% \input{sections/marginal-cost-comparison-neurips}

\textbf{Experimental Baselines.} Few FL mechanisms eliminate the free-rider effect, with none doing so without sharing data.
Therefore, we adapt the mechanism proposed by \citet{karimireddy2022mechanisms} as the baseline to compare against (we denote it as \textsc{Linear} \realfm).
We also compare \realfm to a local training baseline where
we measure the average device utility attained by devices if they did not participate in the mechanism.
Server utility is inferred in this instance by using the average accuracy of locally trained models.

\textbf{Testing Scenarios.} 
We test \realfm and its baselines under homogeneous and heterogeneous device data distributions.
In the heterogeneous case, we use two different Dirichlet distributions (parameters $0.6$ and $0.3$) to determine label proportions for each device \cite{gao2022feddc}.
These settings are denoted as $D-0.6$ and $D-0.3$ respectively.
We also test \realfm under non-uniform marginal costs (C) and accuracy payoffs functions (P).
Due to space constraints, additional experiments and details are in Appendix \ref{app:exp}.

\input{figures/data-contribution-comparison-16}

\textbf{Increased Contributions to Federated Training.}
Figure \ref{fig:data-contribution-comparison-16} showcases the power of \realfm, via its accuracy-shaping function, to incentivize devices to contribute more data points.
Through its construction, \realfm's accuracy-shaping function incentivizes devices to use more data during federated training than locally optimal in exchange for greater utility.
This is important for two reasons. First, incentivizing devices to contribute more than local training proves that the free-rider effect is not taking place.
Second, higher data contribution lead to better-performing models and higher accuracies.
This improves the utility for all participants.
Overall, \realfm is superior at incentivizing contributions compared to state-of-the-art FL mechanisms.

\textbf{Improved Server and Device Utility.}
\realfm leverages an improved reward mechanism (\Eqref{eq:mech}) to boost the amount of contributions to federated training.
The influx of data subsequently increases model performance (detailed in Section \ref{sec:formulation}).
This is backed up empirically: Figure \ref{fig:server-utility-comparsion-16} showcases upwards of \textit{$5$ magnitudes greater server utility} compared to state-of-the-art FL mechanisms.
Devices participating in \realfm also boost utility \textit{by over $5$ magnitudes} (Figure \ref{fig:device-utility-comparsion-16}).
The improvement stems from (i) effective accuracy-shaping by \realfm and (ii) the use of non-linear accuracy payoff functions $\phi$, which more precisely map the benefit derived from an increase in model accuracy.
%\realfm's accuracy-shaping function is defined (Theorem \ref{thm:acc-shaping}) to improve device utility if devices contribute more data than they would locally.
%Incorporating $\phi$ into device utility makes it more realistic and spurs increased data contribution.
%With utilities that grow increasingly great with improved accuracy, devices are incentivized to contribute more data in order to chase higher model accuracy and subsequent utility.

%\realfm is powered by the incentives provided by its accuracy-shaping function. 
%By Theorem \ref{thm:acc-shaping}, devices provably contribute more data when accuracy-shaping occurs.
%As the total amount of data $m$ grows due to the incentives of accuracy shaping, a higher-performing model is trained by the server.
%A higher-performing model results in higher utility for the server (\Eqref{eq:server-utility}).

\textbf{Performance Under Non-Uniformities.}
We find that non-uniform costs and accuracy payoff functions do not affect \realfm performance.
However, as expected, \realfm performance slightly degrades as device datasets become more heterogeneous (Figures \ref{fig:server-utility-comparsion-16} \& \ref{fig:data-contribution-comparison-16}).
In this setting, both local and federated accuracies are lower due to the difficulties of out-of-distribution generalization and model drift.
%\realfm's federated contributions are affected by the collapse in local accuracies (Figure \ref{fig:acc-plots-16}) stemming from heterogeneous distributions.
%When local accuracies decrease, accuracy shaping becomes less effective, as the server desires fewer contributions from devices with distributions particularly different than the true distribution (Remark \ref{remark6:acc-shaping}).
Nevertheless, even under heterogeneous distributions, \realfm greatly outperforms all other baselines under both non-uniform costs and accuracy payoff functions as well as non-uniform (heterogeneous) device data distributions.
\vspace{-3mm}

==> sections/Checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All claims are verified in Sections 4-6
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail in Appendix \ref{app:notation} that we assume devices are honest. At the same time, we provide avenues to combat this issue if it arises in practice.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are listed in the main body of the paper. Proofs are found in Appendix \ref{app:proofs}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Experiment details are listed in Section \ref{sec:experiments} and Appendix \ref{app:exp}. Furthermore, code is provided to ensure reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code is provided to reviewers.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All details are provided in Section \ref{sec:experiments} and Appendix \ref{app:exp}. Furthermore, code is provided to ensure reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All experiments were run 3 trials and error bars can be seen in our plots in Appendix \ref{app:exp}. The majority of our plots use the average results of the three trials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Computational resources are detailed in Appendix \ref{app:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reach the Code of Ethics and have abided by it. Everything submitted is anonymous.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work may not have immense societal impact, yet we include a section about our impact in Appendix \ref{app:impact}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code is provided to reviewers and is documented.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/algo_RealFM-Algorithm.tex <==
\begin{algorithm}[t]
\caption{\realfm: A Realistic Federated Mechanism}
\label{alg:realfm}
\begin{algorithmic}
  \STATE {\bfseries Input:} Data contributions $\bm{m}$, marginal costs $\bm{c}$, profit margin $p_m$, payoff/shaping/accuracy functions $\bm{\phi}$/$\bm{\gamma}$/$\bm{a}$, $h$ local steps, $T$ total iterations, total epochs $E$, initial parameters $\bm{w^1}$, loss $\ell$, and step-size $\eta$.
  \STATE {\bfseries Output:} Model accuracy $a^r_i$ and reward $R_i$.
  \STATE $s_i \leftarrow m_i / \sum_{j=1}^{n} m_j$ %\tcp*{compute self-weight for federated averaging}
  \FOR{$t = 1, \ldots, T$}
    \STATE Server distributes $\bm{w^t}$ to all devices
    \FOR{$h$ local steps, each device $i$ \textbf{in parallel}}
    \STATE $\bm{w_i^{t+1}} \leftarrow$ ClientUpdate($i, \bm{w^t}$)
    \ENDFOR
    \STATE $\bm{w^{t+1}} \leftarrow \sum_j s_j \bm{w_i^{t+1}}$
    \ENDFOR
    \STATE $r(\bm{m}) \leftarrow (1-p_m)\frac{\phi_C\left(a_C\left(\sum_j m_j\right)\right)}{\sum_j m_j}$ % \tcp*{compute monetary reward}
    \FOR{$i = 1$ to $n$}
    \STATE Compute $m_i^o$ and $m_i^*$ using $a_i, c_i, \phi_i$, and $\gamma_i(m_i)$
    \STATE Return $(a^r_i, R_i)$ to device $i$ using Eq. \ref{eq:mech}
    \ENDFOR
    \vspace{0.25\baselineskip}
    \STATE {\bfseries ClientUpdate}($i, \bm{w}$):\;
    $\mathcal{B} \leftarrow$ batch $m_i$ data points\;
     \FOR{each epoch $e = 1, \ldots, E$}
     \FOR{batch $b \in \mathcal{B}$}
     \STATE $\bm{w} \leftarrow \bm{w} - \eta \nabla \ell(\bm{w}; b)$
    \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}


==> sections/fig_marginal-cost-comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/marginal-cost-comparison-fig.pdf}
    \vspace{-2mm}
    \caption{\textbf{Local Optimal Data Contribution for Varying Payoff Functions.} We compare optimal data contribution across different payoff functions. As expected, realistic power payoff functions, $\phi_i(a) = \frac{1}{(1-a)^2} - 1$, result in greater optimal data contribution compared to linear payoff functions, $\phi_i(a) = a$. We define $\hat{a}_i(m)$ as in \Eqref{eq:gen-bound}, with $a_{opt}^i = 0.95$ and multiple values of $k$.}
    \label{fig:cost-comparison}
    \vspace{-1mm}
\end{figure}

==> sections/temp.tex <==
Assumption \ref{assum:a3} simply states that the central server will train a model that at least matches the best performing locally trained model.
This is a mild assumption, as in practice the performance of a model trained using contributions from a wide swath of devices outperforms any model trained locally by one of the same devices.
This assumption is violated only if a device $i$ contributes a large quantity of junk updates (thereby having a low $a_{opt}^i$).
To combat this situation, and avoid any violations in practice, the central server may refuse service to such devices.
Dataset valuation, either via Federated Shapley Values \citep{wang2020principled} or other techniques, is one method to detect such devices.
